Scoped and Typed Staging by Evaluation

Using a dependently typed host language, we give a well scoped-and-typed by construction presentation of a minimal two level simply typed calculus with a static and a dynamic stage. The staging function partially evaluating the part of a term that are static is obtained by a model construction inspired by normalisation by evaluation. We then go on to demonstrate how this minimal language can be extended to provide additional metaprogramming capabilities, and to define a higher order functional language evaluating to digital circuit descriptions.

==> BasicTwoTT.tex <==
\begin{code}%
\>[0]\AgdaSymbol{\{-\#}\AgdaSpace{}%
\AgdaKeyword{OPTIONS}\AgdaSpace{}%
\AgdaPragma{--safe}\AgdaSpace{}%
\AgdaPragma{--without-K}\AgdaSpace{}%
\AgdaSymbol{\#-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{------------------------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ The\ content\ of\ this\ module\ is\ based\ on\ the\ paper}\<%
\\
\>[0]\AgdaComment{--\ Staged\ compilation\ with\ two-level\ type\ theory}\<%
\\
\>[0]\AgdaComment{--\ by\ András\ Kovács}\<%
\\
\>[0]\AgdaComment{--\ https://dl.acm.org/doi/abs/10.1145/3547641}\<%
\\
\>[0]\AgdaComment{--}\<%
\\
\>[0]\AgdaComment{--\ and\ some\ classic\ techniques\ to\ represent\ intrinsically-typed\ calculi}\<%
\\
\>[0]\AgdaComment{------------------------------------------------------------------------}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ This\ is\ the\ stripped\ down\ version\ with\ nothing\ but}\<%
\\
\>[0]\AgdaComment{--\ quotes\ and\ splices!\ See\ TwoTT\ for\ a\ more\ reasonable}\<%
\\
\>[0]\AgdaComment{--\ programming\ langauge.}\<%
\\
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{BasicTwoTT}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Default}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Empty}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{⊥}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Function.Base}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∘\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{id}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{const}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Unary}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{IUniversal}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}⇒\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}⊢\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∩\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{------------------------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ We\ have\ two\ phases:\ source\ code\ and\ staged\ code}\<%
\\
\>[0]\<%
\end{code}
%<*phase>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Phase}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{stg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Phase}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{variable}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Phase}\<%
\end{code}
%</phase>

\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{------------------------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ We\ have\ two\ stages:\ static\ and\ dynamic}\<%
\\
\>[0]\<%
\end{code}
%<*stage>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Phase}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\<%
\\
%
\>[2]\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaGeneralizable{ph}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{variable}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaGeneralizable{ph}\<%
\end{code}
%</stage>
\begin{code}%
\>[0]\AgdaComment{------------------------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ Types\ are\ indexed\ by\ the\ stage\ they\ are\ defined\ at}\<%
\\
\>[0]\AgdaComment{--}\<%
\\
\>[0]\AgdaComment{--\ (⇑\ A)\ is\ the\ static\ representation\ of\ a\ dynamic\ type\ A;\ that\ is}\<%
\\
\>[0]\AgdaComment{--\ to\ say\ it\ is\ morally\ the\ type\ of\ metaprograms\ returning\ code\ of}\<%
\\
\>[0]\AgdaComment{--\ type\ A.}\<%
\\
\>[0]\AgdaComment{--}\<%
\\
\>[0]\AgdaComment{--\ Function\ types\ are\ homogeneous:\ both\ domains\ and\ codomains\ need\ to}\<%
\\
\>[0]\AgdaComment{--\ live\ at\ the\ same\ stage.}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{infixr}\AgdaSpace{}%
\AgdaNumber{5}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}`⇒\AgdaUnderscore{}}}\<%
\\
\>[0]\<%
\end{code}
%<*types>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{`α}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaGeneralizable{st}\<%
\\
%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{`⇑\AgdaUnderscore{}}}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaInductiveConstructor{src}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\<%
\\
%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}`⇒\AgdaUnderscore{}}}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaGeneralizable{st}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{variable}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSpace{}%
\AgdaGeneralizable{C}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaGeneralizable{st}\<%
\end{code}
%</types>
\begin{code}%
\>[0]\<%
\\
\>[0]\<%
\end{code}
%<*asStaged>
\begin{code}%
\>[0]\AgdaFunction{asStaged}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaInductiveConstructor{src}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaInductiveConstructor{stg}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\<%
\\
\>[0]\AgdaFunction{asStaged}\AgdaSpace{}%
\AgdaInductiveConstructor{`α}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`α}\<%
\\
\>[0]\AgdaFunction{asStaged}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{)}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{asStaged}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaFunction{asStaged}\AgdaSpace{}%
\AgdaBound{B}\<%
\end{code}
%</asStaged>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{------------------------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ Context\ are\ your\ usual\ left-nested\ lists\ of\ types.}\<%
\\
\>[0]\AgdaComment{--\ Note\ the\ existential\ quantification\ over\ the\ stage\ of\ the\ freshly}\<%
\\
\>[0]\AgdaComment{--\ bound\ variable\ in\ the\ snoc\ case}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{infixl}\AgdaSpace{}%
\AgdaNumber{4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}\<%
\\
\>[0]\<%
\end{code}
%<*context>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{ε}%
\>[7]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\<%
\\
%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}%
\>[7]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Context}\<%
\end{code}
%</context>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaKeyword{variable}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaGeneralizable{Θ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{------------------------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ Thinnings}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{infix}\AgdaSpace{}%
\AgdaNumber{0}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\<%
\\
\>[0]\<%
\end{code}
%<*thin>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{done}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\<%
\\
%
\>[2]\AgdaInductiveConstructor{keep}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaGeneralizable{A}\<%
\\
%
\>[2]\AgdaInductiveConstructor{drop}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaGeneralizable{A}\<%
\end{code}
%</thin>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Θ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Θ}\<%
\\
\>[0]\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaInductiveConstructor{done}\AgdaSpace{}%
\AgdaInductiveConstructor{done}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{done}\<%
\\
\>[0]\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaBound{p}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaBound{p}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\<%
\\
\>[0]\<%
\end{code}
%<*thinrefl>
\begin{code}%
\>[0]\AgdaFunction{≤-refl}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Γ}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaBound{Γ}\<%
\\
\>[0]\AgdaFunction{≤-refl}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaInductiveConstructor{ε}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{done}\<%
\\
\>[0]\AgdaFunction{≤-refl}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaFunction{≤-refl}\<%
\end{code}
%</thinrefl>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{------------------------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ Variables\ (could\ be\ defined\ as\ thinning\ from\ a\ singleton\ list)}\<%
\\
\>[0]\<%
\end{code}
%<*var>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{here}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}%
\>[23]\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⊢}}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaInductiveConstructor{there}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}%
\>[23]\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},}}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⊢}}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaFunction{]}\<%
\end{code}
%</var>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaFunction{weak-Var}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\<%
\\
\>[0]\AgdaFunction{weak-Var}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Var}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{weak-Var}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\<%
\\
\>[0]\AgdaFunction{weak-Var}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Var}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{------------------------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ Terms\ are\ indexed\ both\ by\ the\ stage\ of\ the\ type\ of\ the\ computation}\<%
\\
\>[0]\AgdaComment{--\ they\ describe\ but\ also\ by\ a\ boolean\ describing\ whether\ it\ is\ legal}\<%
\\
\>[0]\AgdaComment{--\ to\ uses\ quotes\ and\ splices}\<%
\\
\>[0]\<%
\end{code}
%<*term>
%<*termdecl>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[268I]\AgdaSymbol{(}\AgdaBound{ph}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Phase}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaBound{ph}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
\>[.][@{}l@{}]\<[268I]%
\>[12]\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\end{code}
%</termdecl>
%<*termstlc>
\begin{code}%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaInductiveConstructor{`var}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaInductiveConstructor{`app}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaInductiveConstructor{`lam}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⊢}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{]}\<%
\end{code}
%</termstlc>
%<*termtwolevel>
\begin{code}%
%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{`⟨\AgdaUnderscore{}⟩}}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`⇑}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{`∼\AgdaUnderscore{}}}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`⇑}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaFunction{]}\<%
\end{code}
%</termtwolevel>
%</term>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ Action\ of\ thinnings\ on\ terms}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Var}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaBound{b}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{b}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`∼}}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`∼}}\AgdaSpace{}%
\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{------------------------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ Example\ of\ programs}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{WithDefault}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Purely\ dynamic\ identity\ function}\<%
\end{code}
%<*iddyn>
\begin{code}%
\>[0]\AgdaFunction{`idᵈ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
\>[0]\AgdaFunction{`idᵈ}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSymbol{)}\<%
\end{code}
%</iddyn>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ Static\ identity\ function\ for\ dynamic\ values}\<%
\end{code}
%<*idsta>
\begin{code}%
\>[0]\AgdaFunction{`idˢ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
\>[0]\AgdaFunction{`idˢ}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSymbol{)}\<%
\end{code}
%</idsta>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaKeyword{infixr}\AgdaSpace{}%
\AgdaNumber{3}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}`∘\AgdaUnderscore{}}}\<%
\end{code}
%<*composition>
\begin{code}%
\>[0]\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}`∘\AgdaUnderscore{}}}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{B}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{C}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{C}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
\>[0]\AgdaBound{g}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{`∘}}\AgdaSpace{}%
\AgdaBound{f}%
\>[8]\AgdaSymbol{=}%
\>[11]\AgdaKeyword{let}\AgdaSpace{}%
\AgdaBound{Γ≤Γ,A}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaFunction{≤-refl}\AgdaSpace{}%
\AgdaKeyword{in}\<%
\\
%
\>[11]\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{Γ≤Γ,A}\AgdaSpace{}%
\AgdaBound{g}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{Γ≤Γ,A}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSymbol{)))}\<%
\end{code}
%</composition>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{------------------------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ Semantics\ toolkit:\ Kripke\ function\ spaces\ between}\<%
\\
\>[0]\AgdaComment{--\ context-indexed\ type\ families}\<%
\\
\>[0]\<%
\end{code}
%<*kripke>
\begin{code}%
\>[0]\AgdaKeyword{record}\AgdaSpace{}%
\AgdaRecord{□}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Γ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{constructor}\AgdaSpace{}%
\AgdaInductiveConstructor{mkBox}\<%
\\
%
\>[2]\AgdaKeyword{field}\AgdaSpace{}%
\AgdaField{run□}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Δ}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaBound{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{Δ}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Γ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\\
\>[0]\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaRecord{□}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{)}\<%
\end{code}
%</kripke>
\begin{code}%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{□}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Action\ of\ thinnings\ on\ Kripke\ functions\ spaces}\<%
\\
\>[0]\AgdaComment{--\ By\ construction\ they're\ the\ Free\ thinnable}\<%
\\
\>[0]\AgdaFunction{weak-Kripke}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\<%
\\
\>[0]\AgdaFunction{weak-Kripke}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{run□}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{run□}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∘}}\AgdaSpace{}%
\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaBound{σ}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ lambda-abstraction}\<%
\\
\>[0]\AgdaKeyword{infixr}\AgdaSpace{}%
\AgdaNumber{3}\AgdaSpace{}%
\AgdaInductiveConstructor{mkBox}\<%
\end{code}
%<*kripkelam>
\begin{code}%
\>[0]\AgdaKeyword{syntax}\AgdaSpace{}%
\AgdaInductiveConstructor{mkBox}\AgdaSpace{}%
\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{b}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{λλ[}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaInductiveConstructor{,}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaInductiveConstructor{]}\AgdaSpace{}%
\AgdaBound{b}\<%
\end{code}
%</kripkelam>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ application}\<%
\end{code}
%<*kripkeapp>
\begin{code}%
\>[0]\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}\$\$\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\<%
\\
\>[0]\AgdaBound{f}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\$\$}}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{run□}\AgdaSpace{}%
\AgdaFunction{≤-refl}\AgdaSpace{}%
\AgdaBound{t}\<%
\end{code}
%</kripkeapp>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{------------------------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ Definition\ of\ the\ domain\ for\ staging\ by\ evaluation}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat.Base}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{ℕ}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{suc}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaPrimitive{\AgdaUnderscore{}+\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\AgdaSpace{}%
\AgdaSymbol{as}\AgdaSpace{}%
\AgdaModule{Prod}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}×\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\<%
\end{code}
%<*modelstadecl>
\begin{code}%
\>[0]\AgdaFunction{Static}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\end{code}
%</modelstadecl>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ Static\ values\ are\ intepreted\ in\ the\ domain,}\<%
\\
\>[0]\AgdaComment{--\ Dynamic\ ones\ will\ become\ staged\ terms}\<%
\end{code}
%<*model>
\begin{code}%
\>[0]\AgdaFunction{Value}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\\
\>[0]\AgdaFunction{Value}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}%
\>[11]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{Static}\<%
\\
\>[0]\AgdaFunction{Value}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}%
\>[11]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{stg}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∘}}\AgdaSpace{}%
\AgdaFunction{asStaged}\<%
\end{code}
%</model>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ This\ is\ a\ fairly\ standard\ Kripke\ domain}\<%
\end{code}
%<*modelsta>
\begin{code}%
\>[0]\AgdaFunction{Static}\AgdaSpace{}%
\AgdaInductiveConstructor{`α}%
\>[17]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{const}\AgdaSpace{}%
\AgdaFunction{⊥}\<%
\\
\>[0]\AgdaFunction{Static}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`⇑}}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{)}%
\>[17]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaBound{A}\<%
\\
\>[0]\AgdaFunction{Static}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{)}%
\>[17]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Static}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Static}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{)}\<%
\end{code}
%</modelsta>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ Action\ of\ thinnings\ on\ Kripke\ domains}\<%
\\
\>[0]\AgdaFunction{weak-Static}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Static}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Static}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\<%
\\
\>[0]\AgdaFunction{weak-Static}\AgdaSpace{}%
\AgdaInductiveConstructor{`α}%
\>[21]\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{id}\<%
\\
\>[0]\AgdaFunction{weak-Static}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`⇑}}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{)}%
\>[21]\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\<%
\\
\>[0]\AgdaFunction{weak-Static}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{weak-Kripke}\AgdaSpace{}%
\AgdaBound{σ}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Action\ of\ thinnings\ on\ Values}\<%
\\
\>[0]\AgdaFunction{weak-Value}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\<%
\\
\>[0]\AgdaFunction{weak-Value}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{st}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{weak-Static}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
\>[0]\AgdaFunction{weak-Value}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{st}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{------------------------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ Evaluator\ for\ staging\ by\ evaluation}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Type\ of\ environments\ mapping\ variables\ to\ values}\<%
\\
\>[0]\AgdaKeyword{record}\AgdaSpace{}%
\AgdaRecord{Env}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Γ}\AgdaSpace{}%
\AgdaBound{Δ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{field}\AgdaSpace{}%
\AgdaField{get}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{st}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{Δ}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{Env}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Action\ of\ thinnings\ on\ environments}\<%
\\
\>[0]\AgdaComment{--\ (pointwise\ lifting\ of\ the\ action\ on\ values)}\<%
\\
\>[0]\AgdaFunction{weak-Env}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Θ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Env}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Env}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaGeneralizable{Θ}\<%
\\
\>[0]\AgdaFunction{weak-Env}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{get}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{A}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{weak-Value}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{get}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Semantics\ counterpart\ to\ app}\<%
\end{code}
%<*app>
\begin{code}%
\>[0]\AgdaFunction{app}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[766I]\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaBound{st}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
\>[.][@{}l@{}]\<[766I]%
\>[6]\AgdaFunction{Value}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\<%
\\
\>[0]\AgdaFunction{app}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}%
\>[9]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}\$\$\AgdaUnderscore{}}}\<%
\\
\>[0]\AgdaFunction{app}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}%
\>[9]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`app}\<%
\end{code}
%</app>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ Extending\ an\ environment\ with\ a\ value\ to\ push\ it\ under\ a\ binder}\<%
\end{code}
%<*extend>
\begin{code}%
\>[0]\AgdaFunction{extend}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaRecord{Env}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaRecord{□}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Value}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaRecord{Env}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
\>[0]\AgdaFunction{extend}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{run□}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{get}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
\>[0]\AgdaFunction{extend}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{run□}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{get}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{A}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{weak-Value}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{get}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\<%
\\
\>[0]\<%
\end{code}
%</extend>
\begin{code}%
\>[0]\<%
\\
\>[0]\<%
\end{code}
%<*lam>
\begin{code}%
\>[0]\AgdaFunction{lam}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[836I]\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaBound{st}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
\>[.][@{}l@{}]\<[836I]%
\>[6]\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Value}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Value}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
%
\>[6]\AgdaFunction{Value}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\<%
\\
\>[0]\AgdaFunction{lam}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}%
\>[9]\AgdaBound{b}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{λλ[}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaInductiveConstructor{,}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaInductiveConstructor{]}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{run□}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
\>[0]\AgdaFunction{lam}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}%
\>[9]\AgdaBound{b}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{b}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{run□}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaFunction{≤-refl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSymbol{))}\<%
\end{code}
%</lam>

%<*bodydecl>
\begin{code}%
\>[0]\AgdaFunction{body}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[880I]\AgdaRecord{Env}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
\>[.][@{}l@{}]\<[880I]%
\>[7]\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Value}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Value}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\<%
\end{code}
%</bodydecl>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ Evaluation\ function\ turning\ source\ terms\ into\ values\ provided}\<%
\\
\>[0]\AgdaComment{--\ we\ have\ an\ environment\ assigning\ values\ to\ variables}\<%
\end{code}
%<*evaldecl>
\begin{code}%
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{Env}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\<%
\end{code}
%</evaldecl>
%<*eval>
\begin{code}%
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}%
\>[29]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{get}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{st}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{st}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}%
\>[29]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{app}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{st}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{st}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{b}\AgdaSymbol{)}%
\>[29]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{lam}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{body}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{b}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}%
\>[29]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`∼}}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}%
\>[29]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{v}\<%
\end{code}
%</eval>

%<*body>
\begin{code}%
\>[0]\AgdaFunction{body}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{λλ[}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaInductiveConstructor{,}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaInductiveConstructor{]}\AgdaSpace{}%
\AgdaFunction{eval}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{extend}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{run□}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{b}\<%
\end{code}
%</body>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ Special\ case\ of\ evaluation:\ turning\ source\ terms\ into\ staged\ ones}\<%
\\
\>[0]\<%
\end{code}
%<*stagefun>
%<*stagedecl>
\begin{code}%
\>[0]\AgdaFunction{stage}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{stg}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{asStaged}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\<%
\end{code}
%</stagedecl>
\begin{code}%
\>[0]\AgdaFunction{stage}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{eval}\AgdaSpace{}%
\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaKeyword{where}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{get}\AgdaSpace{}%
\AgdaSymbol{())}\<%
\end{code}
%</stagefun>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≡\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{------------------------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ Tests\ for\ the\ staging\ evaluator}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{infix}\AgdaSpace{}%
\AgdaNumber{0}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∋\AgdaUnderscore{}↝\AgdaUnderscore{}}}\<%
\end{code}
%<*stagedto>
\begin{code}%
\>[0]\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∋\AgdaUnderscore{}↝\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[1001I]\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
\>[.][@{}l@{}]\<[1001I]%
\>[8]\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
%
\>[8]\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{stg}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{asStaged}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\\
\>[0]\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∋}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{↝}}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{stage}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{t}\<%
\end{code}
%</stagedto>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ `idˢ\ is\ a\ static\ identity\ and\ thus\ computes}\<%
\end{code}
%<*testid1>
\begin{code}%
\>[0]\AgdaFunction{test-idˢ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaInductiveConstructor{`α}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaInductiveConstructor{`α}%
\>[21]\AgdaOperator{\AgdaFunction{∋}}%
\>[24]\AgdaOperator{\AgdaInductiveConstructor{`∼}}\AgdaSpace{}%
\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaFunction{`idˢ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaFunction{`idᵈ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\<%
\\
%
\>[21]\AgdaOperator{\AgdaFunction{↝}}%
\>[24]\AgdaFunction{`idᵈ}\<%
\\
\>[0]\AgdaFunction{test-idˢ}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\end{code}
%</testid1>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ `idᵈ\ is\ a\ dynamic\ identity\ and\ thus\ stays\ stuck}\<%
\\
\>[0]\AgdaFunction{test-idᵈ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaInductiveConstructor{`α}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaInductiveConstructor{`α}%
\>[21]\AgdaOperator{\AgdaFunction{∋}}%
\>[24]\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaFunction{`idᵈ}\AgdaSpace{}%
\AgdaFunction{`idᵈ}\<%
\\
%
\>[21]\AgdaOperator{\AgdaFunction{↝}}%
\>[24]\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaFunction{`idᵈ}\AgdaSpace{}%
\AgdaFunction{`idᵈ}\<%
\\
\>[0]\AgdaFunction{test-idᵈ}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ We\ can\ mix\ the\ two!}\<%
\\
\>[0]\AgdaFunction{test-idᵈˢ}\AgdaSpace{}%
\AgdaSymbol{:}\<%
\end{code}
%<*testid01>
\begin{code}%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaInductiveConstructor{`α}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaInductiveConstructor{`α}%
\>[12]\AgdaOperator{\AgdaFunction{∋}}%
\>[15]\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaFunction{`idᵈ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`∼}}\AgdaSpace{}%
\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaFunction{`idˢ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaFunction{`idᵈ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{↝}}%
\>[53]\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaFunction{`idᵈ}\AgdaSpace{}%
\AgdaFunction{`idᵈ}\<%
\end{code}
%</testid01>
\begin{code}%
\>[0]\AgdaFunction{test-idᵈˢ}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%


==> MetaCircuit.tex <==
\begin{code}%
\>[0]\AgdaSymbol{\{-\#}\AgdaSpace{}%
\AgdaKeyword{OPTIONS}\AgdaSpace{}%
\AgdaPragma{--safe}\AgdaSpace{}%
\AgdaPragma{--without-K}\AgdaSpace{}%
\AgdaSymbol{\#-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{MetaCircuit}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{Bool}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{if\AgdaUnderscore{}then\AgdaUnderscore{}else\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Empty}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{⊥}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Fin.Base}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{Fin}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{suc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat.Base}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{ℕ}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaPrimitive{\AgdaUnderscore{}+\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Vec.Base}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{Vec}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}∷\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Function.Base}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∘\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{id}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{const}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Unary}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{IUniversal}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}⇒\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}⊢\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Agda.Builtin.FromNat}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Unit.Base}\<%
\\
\>[0]\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat.Literals}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaKeyword{instance}\AgdaSpace{}%
\AgdaFunction{nat}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{Data.Nat.Literals.number}\<%
\\
\>[0]\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Fin.Literals}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaKeyword{instance}\AgdaSpace{}%
\AgdaFunction{fin}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{n}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Data.Fin.Literals.number}\AgdaSpace{}%
\AgdaBound{n}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Phase}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{stg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Phase}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{variable}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Phase}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Phase}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\<%
\\
%
\>[2]\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaGeneralizable{ph}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{variable}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaGeneralizable{ph}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{infixr}\AgdaSpace{}%
\AgdaNumber{3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}`⇒\AgdaUnderscore{}}}\<%
\\
\>[0]\AgdaKeyword{infixr}\AgdaSpace{}%
\AgdaNumber{5}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇑\AgdaUnderscore{}}}\<%
\\
\>[0]\<%
\end{code}
%<*type>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}`⇒\AgdaUnderscore{}}}%
\>[10]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\<%
\\
%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{`⇑\AgdaUnderscore{}}}%
\>[10]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaInductiveConstructor{src}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\<%
\\
%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{`⟨\AgdaUnderscore{}∣\AgdaUnderscore{}⟩}}%
\>[10]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{i}\AgdaSpace{}%
\AgdaBound{o}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaGeneralizable{ph}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\<%
\end{code}
%</type>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{`Bool}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{variable}\AgdaSpace{}%
\AgdaGeneralizable{m}\AgdaSpace{}%
\AgdaGeneralizable{i}\AgdaSpace{}%
\AgdaGeneralizable{o}\AgdaSpace{}%
\AgdaGeneralizable{i₁}\AgdaSpace{}%
\AgdaGeneralizable{o₁}\AgdaSpace{}%
\AgdaGeneralizable{i₂}\AgdaSpace{}%
\AgdaGeneralizable{o₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\<%
\\
\>[0]\AgdaKeyword{variable}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSpace{}%
\AgdaGeneralizable{C}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaGeneralizable{st}\<%
\\
\>[0]\<%
\end{code}
%<*asStaged>
\begin{code}%
\>[0]\AgdaFunction{asStaged}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaInductiveConstructor{src}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaInductiveConstructor{stg}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\<%
\\
\>[0]\AgdaFunction{asStaged}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaBound{i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaBound{o}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaBound{i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaBound{o}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\<%
\end{code}
%</asStaged>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaKeyword{infixl}\AgdaSpace{}%
\AgdaNumber{3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}\<%
\\
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{ε}%
\>[7]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\<%
\\
%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}%
\>[7]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Context}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{variable}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaGeneralizable{Θ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{infix}\AgdaSpace{}%
\AgdaNumber{0}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\<%
\\
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{done}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\<%
\\
%
\>[2]\AgdaInductiveConstructor{keep}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaGeneralizable{A}\<%
\\
%
\>[2]\AgdaInductiveConstructor{drop}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaGeneralizable{A}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Θ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Θ}\<%
\\
\>[0]\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaInductiveConstructor{done}\AgdaSpace{}%
\AgdaInductiveConstructor{done}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{done}\<%
\\
\>[0]\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaBound{p}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaBound{p}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{≤-refl}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Γ}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaBound{Γ}\<%
\\
\>[0]\AgdaFunction{≤-refl}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaInductiveConstructor{ε}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{done}\<%
\\
\>[0]\AgdaFunction{≤-refl}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaFunction{≤-refl}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{here}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}%
\>[23]\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⊢}}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaInductiveConstructor{there}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}%
\>[23]\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},}}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⊢}}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{weak-Var}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\<%
\\
\>[0]\AgdaFunction{weak-Var}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Var}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{weak-Var}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\<%
\\
\>[0]\AgdaFunction{weak-Var}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Var}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ph}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Phase}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaBound{ph}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaComment{--\ stlc}\<%
\\
%
\>[2]\AgdaInductiveConstructor{`var}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaInductiveConstructor{`app}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaInductiveConstructor{`lam}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⊢}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaComment{--\ two\ level}\<%
\\
%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{`⟨\AgdaUnderscore{}⟩}}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`⇑}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{`∼\AgdaUnderscore{}}}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`⇑}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaComment{--\ booleans}\<%
\\
%
\>[2]\AgdaInductiveConstructor{`true}%
\>[10]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaInductiveConstructor{`Bool}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaInductiveConstructor{`false}%
\>[10]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaInductiveConstructor{`Bool}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaInductiveConstructor{`ifte}%
\>[10]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`Bool}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaComment{--\ circuit}\<%
\end{code}
%<*termcircuit>
%<*termcircuitnand>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{`nand}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaFunction{]}\<%
\end{code}
%</termcircuitnand>
%<*termcircuitpar>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{`par}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}%
\>[15]\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaGeneralizable{i₁}%
\>[40]\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaGeneralizable{o₁}%
\>[52]\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\<%
\\
%
\>[15]\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}%
\>[36]\AgdaGeneralizable{i₂}%
\>[40]\AgdaOperator{\AgdaInductiveConstructor{∣}}%
\>[48]\AgdaGeneralizable{o₂}%
\>[52]\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\<%
\\
%
\>[15]\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaGeneralizable{i₁}\AgdaSpace{}%
\AgdaOperator{\AgdaPrimitive{+}}%
\>[36]\AgdaGeneralizable{i₂}%
\>[40]\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaGeneralizable{o₁}\AgdaSpace{}%
\AgdaOperator{\AgdaPrimitive{+}}%
\>[48]\AgdaGeneralizable{o₂}%
\>[52]\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaFunction{]}\<%
\end{code}
%</termcircuitpar>
%<*termcircuitseq>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{`seq}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}%
\>[15]\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaGeneralizable{i}%
\>[33]\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaGeneralizable{m}%
\>[38]\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\<%
\\
%
\>[15]\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaGeneralizable{m}%
\>[33]\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaGeneralizable{o}%
\>[38]\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\<%
\\
%
\>[15]\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaGeneralizable{i}%
\>[33]\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaGeneralizable{o}%
\>[38]\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaFunction{]}\<%
\end{code}
%</termcircuitseq>
%<*termcircuitmix>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{`mix}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Vec}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{Fin}\AgdaSpace{}%
\AgdaGeneralizable{i}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaGeneralizable{o}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaGeneralizable{i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaGeneralizable{o}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaFunction{]}\<%
\end{code}
%</termcircuitmix>

%<*id2>
\begin{code}%
\>[0]\AgdaFunction{`id₂}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[8]\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
\>[0]\AgdaFunction{`id₂}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`mix}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaNumber{0}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\<%
\end{code}
%</id2>

%<*swap>
\begin{code}%
\>[0]\AgdaFunction{`swap}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[9]\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
\>[0]\AgdaFunction{`swap}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`mix}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaNumber{0}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\<%
\end{code}
%</swap>

%<*dup>
\begin{code}%
\>[0]\AgdaFunction{`dup}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[8]\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
\>[0]\AgdaFunction{`dup}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`mix}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaNumber{0}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaNumber{0}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\<%
\end{code}
%</dup>

%<*diag>
\begin{code}%
\>[0]\AgdaFunction{`diag}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`⇑}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇑}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
\>[0]\AgdaFunction{`diag}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaInductiveConstructor{`seq}\AgdaSpace{}%
\AgdaFunction{`dup}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`∼}}\AgdaSpace{}%
\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\<%
\end{code}
%</diag>

%<*not>
\begin{code}%
\>[0]\AgdaFunction{`not}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
\>[0]\AgdaFunction{`not}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`∼}}\AgdaSpace{}%
\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaFunction{`diag}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaInductiveConstructor{`nand}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\<%
\end{code}
%</not>

%<*and>
\begin{code}%
\>[0]\AgdaFunction{`and}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
\>[0]\AgdaFunction{`and}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`seq}\AgdaSpace{}%
\AgdaInductiveConstructor{`nand}\AgdaSpace{}%
\AgdaFunction{`not}\<%
\end{code}
%</and>
\begin{code}%
\>[0]\<%
\\
\>[0]\<%
\end{code}
%<*or>
\begin{code}%
\>[0]\AgdaFunction{`or}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
\>[0]\AgdaFunction{`or}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`seq}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`par}\AgdaSpace{}%
\AgdaFunction{`not}\AgdaSpace{}%
\AgdaFunction{`not}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{`nand}\<%
\end{code}
%</or>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaFunction{`id₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
\>[0]\AgdaFunction{`id₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`mix}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{zero}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\<%
\\
\>[0]\<%
\end{code}
%<*tab>
\begin{code}%
\>[0]\AgdaFunction{`tab}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{((}\AgdaInductiveConstructor{`Bool}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇑}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇑}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
\>[0]\AgdaFunction{`tab}\AgdaSpace{}%
\AgdaSymbol{=}%
\>[665I]\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaInductiveConstructor{`seq}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`seq}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`seq}\<%
\\
\>[665I][@{}l@{\AgdaIndent{0}}]%
\>[9]\AgdaSymbol{(}\AgdaInductiveConstructor{`par}\AgdaSpace{}%
\AgdaFunction{`dup}\AgdaSpace{}%
\AgdaFunction{`dup}\AgdaSymbol{)}\<%
\\
%
\>[9]\AgdaSymbol{(}\AgdaInductiveConstructor{`mix}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaNumber{0}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaNumber{3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)))}\<%
\\
%
\>[9]\AgdaSymbol{(}\AgdaInductiveConstructor{`par}%
\>[681I]\AgdaSymbol{(}\AgdaInductiveConstructor{`seq}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`par}\AgdaSpace{}%
\AgdaFunction{`id₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`∼}}\AgdaSpace{}%
\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{`true}\AgdaSymbol{))}%
\>[62]\AgdaFunction{`and}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[681I]%
\>[15]\AgdaSymbol{(}\AgdaInductiveConstructor{`seq}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`par}\AgdaSpace{}%
\AgdaFunction{`not}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`∼}}\AgdaSpace{}%
\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{`false}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaFunction{`and}\AgdaSymbol{)))}\<%
\\
%
\>[9]\AgdaFunction{`or}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\<%
\end{code}
%</tab>

\begin{code}%
\>[0]\AgdaComment{--\ Action\ of\ thinnings\ on\ terms}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Var}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaBound{b}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{b}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`∼}}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`∼}}\AgdaSpace{}%
\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaInductiveConstructor{`nand}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`nand}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`par}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`par}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`seq}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`seq}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`mix}\AgdaSpace{}%
\AgdaBound{k}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`mix}\AgdaSpace{}%
\AgdaBound{k}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaInductiveConstructor{`true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`true}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaInductiveConstructor{`false}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`true}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaInductiveConstructor{`ifte}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`ifte}\<%
\\
\>[0]\<%
\end{code}
%<*kripke>
\begin{code}%
\>[0]\AgdaKeyword{record}\AgdaSpace{}%
\AgdaRecord{□}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Γ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{constructor}\AgdaSpace{}%
\AgdaInductiveConstructor{mkBox}\<%
\\
%
\>[2]\AgdaKeyword{field}\AgdaSpace{}%
\AgdaField{runBox}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Δ}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaBound{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{Δ}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Γ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\\
\>[0]\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaRecord{□}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{)}\<%
\end{code}
%</kripke>
\begin{code}%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{□}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{weak-Kripke}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\<%
\\
\>[0]\AgdaFunction{weak-Kripke}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{runBox}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{runBox}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∘}}\AgdaSpace{}%
\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaBound{σ}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ lambda-abstraction}\<%
\\
\>[0]\AgdaKeyword{infixr}\AgdaSpace{}%
\AgdaNumber{3}\AgdaSpace{}%
\AgdaInductiveConstructor{mkBox}\<%
\end{code}
%<*kripkelam>
\begin{code}%
\>[0]\AgdaKeyword{syntax}\AgdaSpace{}%
\AgdaInductiveConstructor{mkBox}\AgdaSpace{}%
\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{b}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{λλ[}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaInductiveConstructor{,}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaInductiveConstructor{]}\AgdaSpace{}%
\AgdaBound{b}\<%
\end{code}
%</kripkelam>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ application}\<%
\end{code}
%<*kripkeapp>
\begin{code}%
\>[0]\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}\$\$\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\<%
\\
\>[0]\AgdaBound{f}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\$\$}}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{runBox}\AgdaSpace{}%
\AgdaFunction{≤-refl}\AgdaSpace{}%
\AgdaBound{t}\<%
\end{code}
%</kripkeapp>
\begin{code}%
\>[0]\<%
\\
\>[0]\<%
\end{code}
%<*modelstadecl>
\begin{code}%
\>[0]\AgdaFunction{Static}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\end{code}
%</modelstadecl>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ Static\ values\ are\ intepreted\ in\ the\ domain,}\<%
\\
\>[0]\AgdaComment{--\ Dynamic\ ones\ will\ become\ staged\ terms}\<%
\end{code}
%<*model>
\begin{code}%
\>[0]\AgdaFunction{Value}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\\
\>[0]\AgdaFunction{Value}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}%
\>[11]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{Static}\<%
\\
\>[0]\AgdaFunction{Value}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}%
\>[11]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{stg}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∘}}\AgdaSpace{}%
\AgdaFunction{asStaged}\<%
\end{code}
%</model>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ This\ is\ a\ fairly\ standard\ Kripke\ domain}\<%
\end{code}
%<*modelsta>
\begin{code}%
\>[0]\AgdaFunction{Static}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`⇑}}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{)}%
\>[17]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaBound{A}\<%
\\
\>[0]\AgdaFunction{Static}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{)}%
\>[17]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Static}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Static}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{)}\<%
\end{code}
%</modelsta>
\begin{code}%
\>[0]\AgdaFunction{Static}\AgdaSpace{}%
\AgdaInductiveConstructor{`Bool}%
\>[17]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{const}\AgdaSpace{}%
\AgdaDatatype{Bool}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Action\ of\ thinnings\ on\ Kripke\ domains}\<%
\\
\>[0]\AgdaFunction{weak-Static}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Static}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Static}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\<%
\\
\>[0]\AgdaFunction{weak-Static}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`⇑}}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{)}%
\>[21]\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\<%
\\
\>[0]\AgdaFunction{weak-Static}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{weak-Kripke}\AgdaSpace{}%
\AgdaBound{σ}\<%
\\
\>[0]\AgdaFunction{weak-Static}\AgdaSpace{}%
\AgdaInductiveConstructor{`Bool}%
\>[21]\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{id}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Action\ of\ thinnings\ on\ Values}\<%
\\
\>[0]\AgdaFunction{weak-Value}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\<%
\\
\>[0]\AgdaFunction{weak-Value}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{st}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{weak-Static}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
\>[0]\AgdaFunction{weak-Value}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{st}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Type\ of\ environments\ mapping\ variables\ to\ values}\<%
\\
\>[0]\AgdaKeyword{record}\AgdaSpace{}%
\AgdaRecord{Env}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Γ}\AgdaSpace{}%
\AgdaBound{Δ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{field}\AgdaSpace{}%
\AgdaField{lookup}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{st}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{Δ}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{Env}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Action\ of\ thinnings\ on\ environments}\<%
\\
\>[0]\AgdaComment{--\ (pointwise\ lifting\ of\ the\ action\ on\ values)}\<%
\\
\>[0]\AgdaFunction{weak-Env}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Θ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Env}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Env}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaGeneralizable{Θ}\<%
\\
\>[0]\AgdaFunction{weak-Env}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{lookup}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{A}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{weak-Value}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{lookup}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Extending\ an\ environment\ with\ a\ value\ to\ push\ it\ under\ a\ binder}\<%
\end{code}
%<*extend>
\begin{code}%
\>[0]\AgdaFunction{extend}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaRecord{Env}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaRecord{□}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Value}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaRecord{Env}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
\>[0]\AgdaFunction{extend}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{runBox}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{lookup}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
\>[0]\AgdaFunction{extend}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{runBox}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{lookup}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{A}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{weak-Value}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{lookup}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\<%
\end{code}
%<*bodydecl>
\begin{code}%
\>[0]\AgdaFunction{body}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[1120I]\AgdaRecord{Env}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
\>[.][@{}l@{}]\<[1120I]%
\>[7]\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Value}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Value}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\<%
\end{code}
%</bodydecl>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ Evaluation\ function\ turning\ source\ terms\ into\ values\ provided}\<%
\\
\>[0]\AgdaComment{--\ we\ have\ an\ environment\ assigning\ values\ to\ variables}\<%
\end{code}
%<*evaldecl>
\begin{code}%
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{Env}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\<%
\end{code}
%</evaldecl>
%<*eval>
\begin{code}%
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{lookup}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\$\$}}\AgdaSpace{}%
\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaBound{b}\AgdaSymbol{)}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{body}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{b}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`∼}}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaInductiveConstructor{`nand}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`nand}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`par}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`par}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`seq}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`seq}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`mix}\AgdaSpace{}%
\AgdaBound{k}\AgdaSymbol{)}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`mix}\AgdaSpace{}%
\AgdaBound{k}\<%
\end{code}
%</eval>
\begin{code}%
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaInductiveConstructor{`true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaInductiveConstructor{`false}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`ifte}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{A}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{\})}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{=}%
\>[1233I]\AgdaInductiveConstructor{λλ[}\AgdaSpace{}%
\AgdaBound{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaInductiveConstructor{,}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaInductiveConstructor{]}\AgdaSpace{}%
\AgdaInductiveConstructor{λλ[}\AgdaSpace{}%
\AgdaBound{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaInductiveConstructor{,}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaInductiveConstructor{]}\AgdaSpace{}%
\AgdaInductiveConstructor{λλ[}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaInductiveConstructor{,}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaInductiveConstructor{]}\<%
\\
\>[.][@{}l@{}]\<[1233I]%
\>[4]\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{if}}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{then}}\AgdaSpace{}%
\AgdaFunction{weak-Value}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{else}}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\<%
\end{code}

%<*body>
\begin{code}%
\>[0]\AgdaFunction{body}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{λλ[}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaInductiveConstructor{,}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaInductiveConstructor{]}\AgdaSpace{}%
\AgdaFunction{eval}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{extend}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{runBox}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{b}\<%
\end{code}
%</body>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ Special\ case\ of\ evaluation:\ turning\ source\ terms\ into\ staged\ ones}\<%
\\
\>[0]\<%
\end{code}
%<*stagefun>
%<*stagedecl>
\begin{code}%
\>[0]\AgdaFunction{stage}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{stg}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{asStaged}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\<%
\end{code}
%</stagedecl>
\begin{code}%
\>[0]\AgdaFunction{stage}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{eval}\AgdaSpace{}%
\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaKeyword{where}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{lookup}\AgdaSpace{}%
\AgdaSymbol{())}\<%
\end{code}
%</stagefun>
\begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≡\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{------------------------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ Tests\ for\ the\ staging\ evaluator}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{infix}\AgdaSpace{}%
\AgdaNumber{0}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∋\AgdaUnderscore{}↝\AgdaUnderscore{}}}\<%
\\
\>[0]\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∋\AgdaUnderscore{}↝\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{stg}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{asStaged}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\\
\>[0]\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∋}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{↝}}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{stage}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{testNot}\AgdaSpace{}%
\AgdaSymbol{:}\<%
\end{code}
%<*testNot>
\begin{code}%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∋}}\AgdaSpace{}%
\AgdaFunction{`not}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{↝}}\AgdaSpace{}%
\AgdaInductiveConstructor{`seq}\AgdaSpace{}%
\AgdaFunction{`dup}\AgdaSpace{}%
\AgdaInductiveConstructor{`nand}\<%
\end{code}
%</testNot>
\begin{code}%
\>[0]\AgdaFunction{testNot}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\<%
\end{code}


==> RunMetaCircuit.tex <==
\begin{code}%
\>[0]\AgdaSymbol{\{-\#}\AgdaSpace{}%
\AgdaKeyword{OPTIONS}\AgdaSpace{}%
\AgdaPragma{--safe}\AgdaSpace{}%
\AgdaPragma{--without-K}\AgdaSpace{}%
\AgdaSymbol{\#-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{RunMetaCircuit}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{Bool}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{if\AgdaUnderscore{}then\AgdaUnderscore{}else\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{not}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Empty}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{⊥}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Fin.Base}\AgdaSpace{}%
\AgdaSymbol{as}\AgdaSpace{}%
\AgdaModule{Fin}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{Fin}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{suc}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}↑ˡ\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}↑ʳ\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat.Base}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{ℕ}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{suc}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaPrimitive{\AgdaUnderscore{}+\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product.Base}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},,\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Vec.Base}\AgdaSpace{}%
\AgdaSymbol{as}\AgdaSpace{}%
\AgdaModule{Vec}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{Vec}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}∷\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}++\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{splitAt}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Function.Base}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}\$\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∘\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{id}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{const}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Unary}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{IUniversal}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}⇒\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}⊢\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Agda.Builtin.FromNat}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Unit.Base}\<%
\\
\>[0]\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat.Literals}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaKeyword{instance}\AgdaSpace{}%
\AgdaFunction{nat}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{Data.Nat.Literals.number}\<%
\\
\>[0]\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Fin.Literals}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaKeyword{instance}\AgdaSpace{}%
\AgdaFunction{fin}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{n}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Data.Fin.Literals.number}\AgdaSpace{}%
\AgdaBound{n}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Phase}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{stg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Phase}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{variable}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Phase}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Phase}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\<%
\\
%
\>[2]\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaGeneralizable{ph}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{variable}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaGeneralizable{ph}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{infixr}\AgdaSpace{}%
\AgdaNumber{3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}`⇒\AgdaUnderscore{}}}\<%
\\
\>[0]\AgdaKeyword{infixr}\AgdaSpace{}%
\AgdaNumber{5}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇑\AgdaUnderscore{}}}\<%
\\
\>[0]\<%
\end{code}
%<*type>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}`⇒\AgdaUnderscore{}}}%
\>[10]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\<%
\\
%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{`⇑\AgdaUnderscore{}}}%
\>[10]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaInductiveConstructor{src}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\<%
\\
%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{`⟨\AgdaUnderscore{}∣\AgdaUnderscore{}⟩}}%
\>[10]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{i}\AgdaSpace{}%
\AgdaBound{o}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaGeneralizable{ph}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaGeneralizable{st}\<%
\\
%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{`[\AgdaUnderscore{}]}}%
\>[10]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{n}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\<%
\end{code}
%</type>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{`Bool}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{variable}\AgdaSpace{}%
\AgdaGeneralizable{m}\AgdaSpace{}%
\AgdaGeneralizable{n}\AgdaSpace{}%
\AgdaGeneralizable{i}\AgdaSpace{}%
\AgdaGeneralizable{o}\AgdaSpace{}%
\AgdaGeneralizable{i₁}\AgdaSpace{}%
\AgdaGeneralizable{o₁}\AgdaSpace{}%
\AgdaGeneralizable{i₂}\AgdaSpace{}%
\AgdaGeneralizable{o₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\<%
\\
\>[0]\AgdaKeyword{variable}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSpace{}%
\AgdaGeneralizable{C}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaGeneralizable{st}\<%
\\
\>[0]\<%
\end{code}
%<*asStaged>
\begin{code}%
\>[0]\AgdaFunction{asStaged}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaInductiveConstructor{src}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaInductiveConstructor{stg}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\<%
\\
\>[0]\AgdaFunction{asStaged}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaBound{i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaBound{o}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaBound{i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaBound{o}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\<%
\end{code}
%</asStaged>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaKeyword{infixl}\AgdaSpace{}%
\AgdaNumber{3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}\<%
\\
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{ε}%
\>[7]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\<%
\\
%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}%
\>[7]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Context}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{variable}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaGeneralizable{Θ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{infix}\AgdaSpace{}%
\AgdaNumber{0}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\<%
\\
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{done}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\<%
\\
%
\>[2]\AgdaInductiveConstructor{keep}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaGeneralizable{A}\<%
\\
%
\>[2]\AgdaInductiveConstructor{drop}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaGeneralizable{A}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Θ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Θ}\<%
\\
\>[0]\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaInductiveConstructor{done}\AgdaSpace{}%
\AgdaInductiveConstructor{done}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{done}\<%
\\
\>[0]\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaBound{p}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaBound{p}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{≤-refl}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Γ}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaBound{Γ}\<%
\\
\>[0]\AgdaFunction{≤-refl}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaInductiveConstructor{ε}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{done}\<%
\\
\>[0]\AgdaFunction{≤-refl}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaFunction{≤-refl}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{here}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}%
\>[23]\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⊢}}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaInductiveConstructor{there}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}%
\>[23]\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},}}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⊢}}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{weak-Var}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\<%
\\
\>[0]\AgdaFunction{weak-Var}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Var}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{weak-Var}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\<%
\\
\>[0]\AgdaFunction{weak-Var}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Var}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ph}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Phase}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaBound{ph}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaComment{--\ stlc}\<%
\\
%
\>[2]\AgdaInductiveConstructor{`var}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaInductiveConstructor{`app}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaInductiveConstructor{`lam}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⊢}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaComment{--\ two\ level}\<%
\\
%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{`⟨\AgdaUnderscore{}⟩}}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`⇑}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{`∼\AgdaUnderscore{}}}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`⇑}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaFunction{]}\<%
\end{code}
%<*runtab>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{`run}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaGeneralizable{i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaGeneralizable{o}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`[}}\AgdaSpace{}%
\AgdaGeneralizable{i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{]}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`[}}\AgdaSpace{}%
\AgdaGeneralizable{o}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{]}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaInductiveConstructor{`tab}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`[}}\AgdaSpace{}%
\AgdaGeneralizable{i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{]}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`[}}\AgdaSpace{}%
\AgdaGeneralizable{o}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{]}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaGeneralizable{i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaGeneralizable{o}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaFunction{]}\<%
\end{code}
%</runtab>
\begin{code}%
%
\>[2]\AgdaComment{--\ booleans}\<%
\\
%
\>[2]\AgdaInductiveConstructor{`true}%
\>[10]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaInductiveConstructor{`Bool}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaInductiveConstructor{`false}%
\>[10]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaInductiveConstructor{`Bool}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaInductiveConstructor{`ifte}%
\>[10]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`Bool}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaComment{--\ vectors}\<%
\\
%
\>[2]\AgdaInductiveConstructor{`nil}%
\>[10]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`[}}\AgdaSpace{}%
\AgdaNumber{0}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{]}}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaInductiveConstructor{`cons}%
\>[10]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`Bool}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`[}}\AgdaSpace{}%
\AgdaGeneralizable{n}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{]}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`[}}\AgdaSpace{}%
\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaGeneralizable{n}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{]}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaInductiveConstructor{`split}%
\>[10]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{((}\AgdaInductiveConstructor{`Bool}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`[}}\AgdaSpace{}%
\AgdaGeneralizable{n}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{]}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`[}}\AgdaSpace{}%
\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaGeneralizable{n}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{]}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaComment{--\ circuit}\<%
\end{code}
%<*termcircuit>
%<*termcircuitconstant>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{`const}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Bool}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaNumber{0}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaFunction{]}\<%
\end{code}
%<*termcircuitnand>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{`nand}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaFunction{]}\<%
\end{code}
%</termcircuitnand>
%<*termcircuitpar>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{`par}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}%
\>[15]\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaGeneralizable{i₁}%
\>[40]\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaGeneralizable{o₁}%
\>[52]\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\<%
\\
%
\>[15]\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}%
\>[36]\AgdaGeneralizable{i₂}%
\>[40]\AgdaOperator{\AgdaInductiveConstructor{∣}}%
\>[48]\AgdaGeneralizable{o₂}%
\>[52]\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\<%
\\
%
\>[15]\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaGeneralizable{i₁}\AgdaSpace{}%
\AgdaOperator{\AgdaPrimitive{+}}%
\>[36]\AgdaGeneralizable{i₂}%
\>[40]\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaGeneralizable{o₁}\AgdaSpace{}%
\AgdaOperator{\AgdaPrimitive{+}}%
\>[48]\AgdaGeneralizable{o₂}%
\>[52]\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaFunction{]}\<%
\end{code}
%</termcircuitpar>
%<*termcircuitseq>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{`seq}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}%
\>[15]\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaGeneralizable{i}%
\>[33]\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaGeneralizable{m}%
\>[38]\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\<%
\\
%
\>[15]\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaGeneralizable{m}%
\>[33]\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaGeneralizable{o}%
\>[38]\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\<%
\\
%
\>[15]\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaGeneralizable{i}%
\>[33]\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaGeneralizable{o}%
\>[38]\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaFunction{]}\<%
\end{code}
%</termcircuitseq>
%<*termcircuitmix>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{`mix}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Vec}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{Fin}\AgdaSpace{}%
\AgdaGeneralizable{i}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaGeneralizable{o}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaGeneralizable{i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaGeneralizable{o}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaFunction{]}\<%
\end{code}
%</termcircuitmix>

%<*id2>
\begin{code}%
\>[0]\AgdaFunction{`id₂}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[8]\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
\>[0]\AgdaFunction{`id₂}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`mix}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaNumber{0}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\<%
\end{code}
%</id2>

%<*swap>
\begin{code}%
\>[0]\AgdaFunction{`swap}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[9]\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
\>[0]\AgdaFunction{`swap}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`mix}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaNumber{0}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\<%
\end{code}
%</swap>

%<*dup>
\begin{code}%
\>[0]\AgdaFunction{`dup}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[8]\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
\>[0]\AgdaFunction{`dup}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`mix}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaNumber{0}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaNumber{0}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\<%
\end{code}
%</dup>

%<*diag>
\begin{code}%
\>[0]\AgdaFunction{`diag}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`⇑}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇑}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
\>[0]\AgdaFunction{`diag}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaInductiveConstructor{`seq}\AgdaSpace{}%
\AgdaFunction{`dup}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`∼}}\AgdaSpace{}%
\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\<%
\end{code}
%</diag>

%<*not>
\begin{code}%
\>[0]\AgdaFunction{`not}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
\>[0]\AgdaFunction{`not}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`seq}\AgdaSpace{}%
\AgdaFunction{`dup}\AgdaSpace{}%
\AgdaInductiveConstructor{`nand}\<%
\end{code}
%</not>

%<*and>
\begin{code}%
\>[0]\AgdaFunction{`and}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
\>[0]\AgdaFunction{`and}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`seq}\AgdaSpace{}%
\AgdaInductiveConstructor{`nand}\AgdaSpace{}%
\AgdaFunction{`not}\<%
\end{code}
%</and>
\begin{code}%
\>[0]\<%
\\
\>[0]\<%
\end{code}
%<*or>
\begin{code}%
\>[0]\AgdaFunction{`or}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
\>[0]\AgdaFunction{`or}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`seq}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`par}\AgdaSpace{}%
\AgdaFunction{`not}\AgdaSpace{}%
\AgdaFunction{`not}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{`nand}\<%
\end{code}
%</or>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaFunction{`id₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
\>[0]\AgdaFunction{`id₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`mix}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{zero}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Action\ of\ thinnings\ on\ terms}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Var}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaBound{b}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{b}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`∼}}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`∼}}\AgdaSpace{}%
\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`run}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`run}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`tab}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`tab}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`const}\AgdaSpace{}%
\AgdaBound{b}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`const}\AgdaSpace{}%
\AgdaBound{b}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaInductiveConstructor{`nand}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`nand}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`par}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`par}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`seq}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`seq}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`mix}\AgdaSpace{}%
\AgdaBound{k}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`mix}\AgdaSpace{}%
\AgdaBound{k}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaInductiveConstructor{`true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`true}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaInductiveConstructor{`false}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`true}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaInductiveConstructor{`ifte}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`ifte}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaInductiveConstructor{`nil}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`nil}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaInductiveConstructor{`cons}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`cons}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaInductiveConstructor{`split}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`split}\<%
\\
\>[0]\<%
\end{code}
%<*kripke>
\begin{code}%
\>[0]\AgdaKeyword{record}\AgdaSpace{}%
\AgdaRecord{□}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Γ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{constructor}\AgdaSpace{}%
\AgdaInductiveConstructor{mkBox}\<%
\\
%
\>[2]\AgdaKeyword{field}\AgdaSpace{}%
\AgdaField{runBox}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Δ}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaBound{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{Δ}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Γ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\\
\>[0]\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaRecord{□}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{)}\<%
\end{code}
%</kripke>
\begin{code}%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{□}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{weak-Kripke}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\<%
\\
\>[0]\AgdaFunction{weak-Kripke}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{runBox}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{runBox}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∘}}\AgdaSpace{}%
\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaBound{σ}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ lambda-abstraction}\<%
\\
\>[0]\AgdaKeyword{infixr}\AgdaSpace{}%
\AgdaNumber{3}\AgdaSpace{}%
\AgdaInductiveConstructor{mkBox}\<%
\end{code}
%<*kripkelam>
\begin{code}%
\>[0]\AgdaKeyword{syntax}\AgdaSpace{}%
\AgdaInductiveConstructor{mkBox}\AgdaSpace{}%
\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{b}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{λλ[}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaInductiveConstructor{,}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaInductiveConstructor{]}\AgdaSpace{}%
\AgdaBound{b}\<%
\end{code}
%</kripkelam>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ application}\<%
\end{code}
%<*kripkeapp>
\begin{code}%
\>[0]\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}\$\$\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\<%
\\
\>[0]\AgdaBound{f}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\$\$}}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{runBox}\AgdaSpace{}%
\AgdaFunction{≤-refl}\AgdaSpace{}%
\AgdaBound{t}\<%
\end{code}
%</kripkeapp>
\begin{code}%
\>[0]\<%
\\
\>[0]\<%
\end{code}
%<*modelstadecl>
\begin{code}%
\>[0]\AgdaFunction{Static}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\end{code}
%</modelstadecl>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ Static\ values\ are\ intepreted\ in\ the\ domain,}\<%
\\
\>[0]\AgdaComment{--\ Dynamic\ ones\ will\ become\ staged\ terms}\<%
\end{code}
%<*model>
\begin{code}%
\>[0]\AgdaFunction{Value}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\\
\>[0]\AgdaFunction{Value}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}%
\>[11]\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{Static}\AgdaSpace{}%
\AgdaBound{A}\<%
\\
\>[0]\AgdaFunction{Value}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}%
\>[11]\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{stg}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{asStaged}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\<%
\end{code}
%</model>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ This\ is\ a\ fairly\ standard\ Kripke\ domain}\<%
\end{code}
%<*modelsta>
\begin{code}%
\>[0]\AgdaFunction{Static}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`⇑}}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{)}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaBound{A}\<%
\\
\>[0]\AgdaFunction{Static}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{)}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{Static}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Static}\AgdaSpace{}%
\AgdaBound{B}\<%
\end{code}
%</modelsta>
\begin{code}%
\>[0]\AgdaFunction{Static}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaBound{i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaBound{o}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{stg}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaBound{i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaBound{o}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\<%
\\
\>[0]\AgdaFunction{Static}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`[}}\AgdaSpace{}%
\AgdaBound{n}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{]}}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{Vec}\AgdaSpace{}%
\AgdaDatatype{Bool}\AgdaSpace{}%
\AgdaBound{n}\<%
\\
\>[0]\AgdaFunction{Static}\AgdaSpace{}%
\AgdaInductiveConstructor{`Bool}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{Bool}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Type\ of\ environments\ mapping\ variables\ to\ values}\<%
\\
\>[0]\AgdaKeyword{record}\AgdaSpace{}%
\AgdaRecord{Env}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Γ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{field}\AgdaSpace{}%
\AgdaField{lookup}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{st}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaBound{A}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{Env}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Extending\ an\ environment\ with\ a\ value\ to\ push\ it\ under\ a\ binder}\<%
\end{code}
%<*extend>
\begin{code}%
\>[0]\AgdaFunction{extend}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{Env}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Env}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{extend}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{lookup}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
\>[0]\AgdaFunction{extend}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{lookup}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{lookup}\AgdaSpace{}%
\AgdaBound{x}\<%
\end{code}
%<*bodydecl>
\begin{code}%
\>[0]\AgdaFunction{body}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[1127I]\AgdaRecord{Env}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
\>[.][@{}l@{}]\<[1127I]%
\>[7]\AgdaFunction{Value}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{B}\<%
\end{code}
%</bodydecl>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaOperator{\AgdaFunction{≈\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{stg}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaGeneralizable{i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaGeneralizable{o}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Vec}\AgdaSpace{}%
\AgdaDatatype{Bool}\AgdaSpace{}%
\AgdaGeneralizable{i}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Vec}\AgdaSpace{}%
\AgdaDatatype{Bool}\AgdaSpace{}%
\AgdaGeneralizable{o}\<%
\\
\>[0]\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{≈}}\AgdaSpace{}%
\AgdaInductiveConstructor{`const}\AgdaSpace{}%
\AgdaBound{b}\AgdaSymbol{)}%
\>[14]\AgdaBound{vs}%
\>[28]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
\>[0]\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{≈}}\AgdaSpace{}%
\AgdaInductiveConstructor{`nand}\AgdaSymbol{)}%
\>[14]\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{y}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}%
\>[28]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{not}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∧}}\AgdaSpace{}%
\AgdaBound{y}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
\>[0]\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{≈}}\AgdaSpace{}%
\AgdaInductiveConstructor{`seq}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}%
\>[14]\AgdaBound{vs}%
\>[28]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaKeyword{let}\AgdaSpace{}%
\AgdaBound{ws}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{≈}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{vs}\AgdaSpace{}%
\AgdaKeyword{in}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{≈}}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ws}\<%
\\
\>[0]\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{≈}}\AgdaSpace{}%
\AgdaInductiveConstructor{`mix}\AgdaSpace{}%
\AgdaBound{c}\AgdaSymbol{)}%
\>[14]\AgdaBound{vs}%
\>[28]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{Vec.map}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Vec.lookup}\AgdaSpace{}%
\AgdaBound{vs}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{c}\<%
\\
\>[0]\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{≈}}\AgdaSpace{}%
\AgdaInductiveConstructor{`par}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}%
\>[14]\AgdaBound{vs}%
\>[28]\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{let}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{vsₗ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,,}}\AgdaSpace{}%
\AgdaBound{vsᵣ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{splitAt}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{vs}\AgdaSpace{}%
\AgdaKeyword{in}\<%
\\
%
\>[2]\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{≈}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{vsₗ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{++}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{≈}}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{vsᵣ}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{tabulate}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Vec}\AgdaSpace{}%
\AgdaDatatype{Bool}\AgdaSpace{}%
\AgdaGeneralizable{o}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{stg}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaNumber{0}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaGeneralizable{o}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\<%
\\
\>[0]\AgdaFunction{tabulate}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{o}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSymbol{\}}%
\>[21]\AgdaBound{vs}%
\>[31]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`mix}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
\>[0]\AgdaFunction{tabulate}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{o}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{o}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{v}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{vs}\AgdaSymbol{)}%
\>[31]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`par}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`const}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{tabulate}\AgdaSpace{}%
\AgdaBound{vs}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{replicateₙ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{o}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{stg}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaBound{o}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\<%
\\
\>[0]\AgdaFunction{replicateₙ}\AgdaSpace{}%
\AgdaBound{o}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`mix}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Vec.replicate}\AgdaSpace{}%
\AgdaBound{o}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{duplicateₙ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{i}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{stg}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaBound{i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaBound{i}\AgdaSpace{}%
\AgdaOperator{\AgdaPrimitive{+}}\AgdaSpace{}%
\AgdaBound{i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\<%
\\
\>[0]\AgdaFunction{duplicateₙ}\AgdaSpace{}%
\AgdaBound{i}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaKeyword{let}\AgdaSpace{}%
\AgdaBound{all}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{Vec.allFin}\AgdaSpace{}%
\AgdaBound{i}\AgdaSpace{}%
\AgdaKeyword{in}\AgdaSpace{}%
\AgdaInductiveConstructor{`mix}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{all}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{++}}\AgdaSpace{}%
\AgdaBound{all}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{double}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ℕ}\<%
\\
\>[0]\AgdaFunction{double}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\<%
\\
\>[0]\AgdaFunction{double}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{n}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSpace{}%
\AgdaOperator{\AgdaPrimitive{+}}\AgdaSpace{}%
\AgdaFunction{double}\AgdaSpace{}%
\AgdaBound{n}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{interleaveₙ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{i}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{stg}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaBound{i}\AgdaSpace{}%
\AgdaOperator{\AgdaPrimitive{+}}\AgdaSpace{}%
\AgdaBound{i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaFunction{double}\AgdaSpace{}%
\AgdaBound{i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\<%
\\
\>[0]\AgdaFunction{interleaveₙ}\AgdaSpace{}%
\AgdaNumber{0}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`mix}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
\>[0]\AgdaFunction{interleaveₙ}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`mix}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Vec.allFin}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaCatchallClause{\AgdaFunction{interleaveₙ}}\AgdaSpace{}%
\AgdaCatchallClause{\AgdaSymbol{(}}\AgdaCatchallClause{\AgdaInductiveConstructor{suc}}\AgdaSpace{}%
\AgdaCatchallClause{\AgdaBound{i}}\AgdaCatchallClause{\AgdaSymbol{)}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaKeyword{let}\AgdaSpace{}%
\AgdaBound{[1⋯i]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{Vec.tail}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\$}}\AgdaSpace{}%
\AgdaFunction{Vec.allFin}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{i}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{in}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{`seq}%
\>[1347I]\AgdaSymbol{(}\AgdaInductiveConstructor{`mix}%
\>[1348I]\AgdaSymbol{(}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{zero}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{↑ˡ}}\AgdaSpace{}%
\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{i}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[1348I]%
\>[13]\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{i}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{↑ʳ}}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSymbol{)}\<%
\\
%
\>[13]\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaFunction{Vec.map}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}↑ˡ}}\AgdaSpace{}%
\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{i}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{[1⋯i]}\<%
\\
\>[1347I][@{}l@{\AgdaIndent{0}}]%
\>[12]\AgdaOperator{\AgdaFunction{++}}\AgdaSpace{}%
\AgdaFunction{Vec.map}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{i}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{↑ʳ\AgdaUnderscore{}}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{[1⋯i]}\AgdaSymbol{))}\<%
\\
\>[.][@{}l@{}]\<[1347I]%
\>[7]\AgdaSymbol{(}\AgdaInductiveConstructor{`par}\AgdaSpace{}%
\AgdaFunction{`id₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{interleaveₙ}\AgdaSpace{}%
\AgdaBound{i}\AgdaSymbol{))}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{zipWithₙ}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[1371I]\AgdaSymbol{(}\AgdaBound{i}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{stg}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
\>[.][@{}l@{}]\<[1371I]%
\>[11]\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{stg}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaFunction{double}\AgdaSpace{}%
\AgdaBound{i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaBound{i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\<%
\\
\>[0]\AgdaFunction{zipWithₙ}\AgdaSpace{}%
\AgdaNumber{0}%
\>[17]\AgdaBound{op}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`mix}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
\>[0]\AgdaFunction{zipWithₙ}\AgdaSpace{}%
\AgdaNumber{1}%
\>[17]\AgdaBound{op}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{op}\<%
\\
\>[0]\AgdaCatchallClause{\AgdaFunction{zipWithₙ}}\AgdaSpace{}%
\AgdaCatchallClause{\AgdaSymbol{(}}\AgdaCatchallClause{\AgdaInductiveConstructor{suc}}\AgdaSpace{}%
\AgdaCatchallClause{\AgdaBound{i}}\AgdaCatchallClause{\AgdaSymbol{)}}\AgdaSpace{}%
\AgdaCatchallClause{\AgdaBound{op}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`par}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{zipWithₙ}\AgdaSpace{}%
\AgdaBound{i}\AgdaSpace{}%
\AgdaBound{op}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{pointwiseₙ}\AgdaSpace{}%
\AgdaSymbol{:}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{(}\AgdaBound{op}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{stg}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
%
\>[4]\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{stg}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaGeneralizable{i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaGeneralizable{o}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
%
\>[4]\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{stg}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaGeneralizable{i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaGeneralizable{o}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\<%
\\
\>[0]\AgdaFunction{pointwiseₙ}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{i}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{o}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`seq}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{duplicateₙ}\AgdaSpace{}%
\AgdaBound{i}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaOperator{\AgdaFunction{\$}}\AgdaSpace{}%
\AgdaInductiveConstructor{`seq}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`par}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaOperator{\AgdaFunction{\$}}\AgdaSpace{}%
\AgdaInductiveConstructor{`seq}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{interleaveₙ}\AgdaSpace{}%
\AgdaBound{o}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaOperator{\AgdaFunction{\$}}\AgdaSpace{}%
\AgdaFunction{zipWithₙ}\AgdaSpace{}%
\AgdaBound{o}\AgdaSpace{}%
\AgdaBound{op}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaOperator{\AgdaFunction{⟪\AgdaUnderscore{}⟫}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{Vec}\AgdaSpace{}%
\AgdaDatatype{Bool}\AgdaSpace{}%
\AgdaGeneralizable{i}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Vec}\AgdaSpace{}%
\AgdaDatatype{Bool}\AgdaSpace{}%
\AgdaGeneralizable{o}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{stg}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaGeneralizable{i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaGeneralizable{o}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\<%
\\
\>[0]\AgdaOperator{\AgdaFunction{⟪\AgdaUnderscore{}⟫}}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{i}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaNumber{0}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{tabulate}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{f}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaOperator{\AgdaFunction{⟪\AgdaUnderscore{}⟫}}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{i}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{i}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{o}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{o}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{f}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{=}%
\>[1494I]\AgdaKeyword{let}\AgdaSpace{}%
\AgdaBound{[1⋯i]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{Vec.tail}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\$}}\AgdaSpace{}%
\AgdaFunction{Vec.allFin}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{i}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{in}\<%
\\
\>[.][@{}l@{}]\<[1494I]%
\>[4]\AgdaFunction{pointwiseₙ}\AgdaSpace{}%
\AgdaFunction{`or}\<%
\\
\>[4][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{(}\AgdaFunction{pointwiseₙ}\AgdaSpace{}%
\AgdaFunction{`and}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`seq}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`mix}\AgdaSpace{}%
\AgdaBound{[1⋯i]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟪}}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∘}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷\AgdaUnderscore{}}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟫}}\AgdaSymbol{)}\<%
\\
\>[6][@{}l@{\AgdaIndent{0}}]%
\>[8]\AgdaSymbol{(}\AgdaInductiveConstructor{`seq}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`mix}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{zero}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))}%
\>[44]\AgdaSymbol{(}\AgdaFunction{replicateₙ}\AgdaSpace{}%
\AgdaBound{o}\AgdaSymbol{)))}\<%
\\
%
\>[6]\AgdaSymbol{(}\AgdaFunction{pointwiseₙ}\AgdaSpace{}%
\AgdaFunction{`and}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`seq}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`mix}\AgdaSpace{}%
\AgdaBound{[1⋯i]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟪}}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∘}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷\AgdaUnderscore{}}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟫}}\AgdaSymbol{)}\<%
\\
\>[6][@{}l@{\AgdaIndent{0}}]%
\>[8]\AgdaSymbol{(}\AgdaInductiveConstructor{`seq}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`mix}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{zero}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`seq}\AgdaSpace{}%
\AgdaFunction{`not}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{replicateₙ}\AgdaSpace{}%
\AgdaBound{o}\AgdaSymbol{))))}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{cast}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{stg}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaGeneralizable{i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaGeneralizable{o}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaGeneralizable{i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaGeneralizable{o}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\<%
\\
\>[0]\AgdaFunction{cast}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
\>[0]\AgdaFunction{cast}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Evaluation\ function\ turning\ source\ terms\ into\ values\ provided}\<%
\\
\>[0]\AgdaComment{--\ we\ have\ an\ environment\ assigning\ values\ to\ variables}\<%
\end{code}
%<*evaldecl>
\begin{code}%
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{Env}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{A}\<%
\end{code}
%</evaldecl>
%<*eval>
\begin{code}%
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{lookup}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaBound{b}\AgdaSymbol{)}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{body}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{b}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`∼}}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`run}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{≈}}\AgdaSpace{}%
\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`tab}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{st}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{st}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{cast}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟪}}\AgdaSpace{}%
\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟫}}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`const}\AgdaSpace{}%
\AgdaBound{b}\AgdaSymbol{)}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`const}\AgdaSpace{}%
\AgdaBound{b}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaInductiveConstructor{`nand}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`nand}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`par}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`par}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`seq}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`seq}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`mix}\AgdaSpace{}%
\AgdaBound{k}\AgdaSymbol{)}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`mix}\AgdaSpace{}%
\AgdaBound{k}\<%
\end{code}
%</eval>
\begin{code}%
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaInductiveConstructor{`true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaInductiveConstructor{`false}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaInductiveConstructor{`ifte}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{if\AgdaUnderscore{}then\AgdaUnderscore{}else\AgdaUnderscore{}}}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaInductiveConstructor{`nil}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaInductiveConstructor{`cons}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}∷\AgdaUnderscore{}}}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaInductiveConstructor{`split}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{k}\AgdaSpace{}%
\AgdaBound{vvs}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{k}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Vec.head}\AgdaSpace{}%
\AgdaBound{vvs}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Vec.tail}\AgdaSpace{}%
\AgdaBound{vvs}\AgdaSymbol{)}\<%
\end{code}

%<*body>
\begin{code}%
\>[0]\AgdaFunction{body}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{eval}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{extend}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{b}\<%
\end{code}
%</body>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ Special\ case\ of\ evaluation:\ turning\ source\ terms\ into\ staged\ ones}\<%
\\
\>[0]\<%
\end{code}
%<*stagefun>
%<*stagedecl>
\begin{code}%
\>[0]\AgdaFunction{stage}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{stg}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{asStaged}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\<%
\end{code}
%</stagedecl>
\begin{code}%
\>[0]\AgdaFunction{stage}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{eval}\AgdaSpace{}%
\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaKeyword{where}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{lookup}\AgdaSpace{}%
\AgdaSymbol{())}\<%
\end{code}
%</stagefun>
\begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≡\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{------------------------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ Tests\ for\ the\ staging\ evaluator}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{infix}\AgdaSpace{}%
\AgdaNumber{0}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∋\AgdaUnderscore{}↝\AgdaUnderscore{}}}\<%
\\
\>[0]\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∋\AgdaUnderscore{}↝\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{stg}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{asStaged}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\\
\>[0]\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∋}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{↝}}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{stage}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{testNot}\AgdaSpace{}%
\AgdaSymbol{:}\<%
\end{code}
%<*testNot>
\begin{code}%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∋}}\AgdaSpace{}%
\AgdaFunction{`not}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{↝}}\AgdaSpace{}%
\AgdaInductiveConstructor{`seq}\AgdaSpace{}%
\AgdaFunction{`dup}\AgdaSpace{}%
\AgdaInductiveConstructor{`nand}\<%
\end{code}
%</testNot>
\begin{code}%
\>[0]\AgdaFunction{testNot}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{testSwap}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[1783I]\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∣}}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\<%
\\
\>[.][@{}l@{}]\<[1783I]%
\>[11]\AgdaOperator{\AgdaFunction{∋}}\AgdaSpace{}%
\AgdaInductiveConstructor{`tab}%
\>[1789I]\AgdaSymbol{(}\AgdaSpace{}%
\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaInductiveConstructor{`split}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\$}}\AgdaSpace{}%
\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaComment{\{-\ x\ -\}}\<%
\\
\>[.][@{}l@{}]\<[1789I]%
\>[18]\AgdaOperator{\AgdaFunction{\$}}\AgdaSpace{}%
\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaInductiveConstructor{`split}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\$}}\AgdaSpace{}%
\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaComment{\{-\ y\ -\}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\$}}\AgdaSpace{}%
\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaComment{\{-\ []\ -\}}\<%
\\
%
\>[18]\AgdaOperator{\AgdaFunction{\$}}\AgdaSpace{}%
\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaInductiveConstructor{`cons}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSymbol{)))}\<%
\\
%
\>[18]\AgdaOperator{\AgdaFunction{\$}}\AgdaSpace{}%
\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaInductiveConstructor{`cons}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSymbol{))))}\<%
\\
%
\>[18]\AgdaOperator{\AgdaFunction{\$}}\AgdaSpace{}%
\AgdaInductiveConstructor{`nil}\AgdaSymbol{)}\<%
\\
%
\>[11]\AgdaOperator{\AgdaFunction{↝}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\<%
\\
\>[0]\AgdaFunction{testSwap}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\end{code}


==> STLC.tex <==
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{STLC}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Function.Base}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∘\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}×\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Agda.Builtin.Equality}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≡\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{infixr}\AgdaSpace{}%
\AgdaNumber{5}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}`⇒\AgdaUnderscore{}}}\<%
\end{code}
%<*type>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{`α}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\<%
\\
%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}`⇒\AgdaUnderscore{}}}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\<%
\end{code}
%</type>
\begin{code}%
\>[0]\<%
\\
\>[0]\<%
\end{code}
%<*typevariables>
\begin{code}%
\>[0]\AgdaKeyword{variable}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSpace{}%
\AgdaGeneralizable{C}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\<%
\end{code}
%</typevariables>
\begin{code}%
\>[0]\<%
\\
\>[0]\<%
\end{code}
%<*context>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{ε}%
\>[7]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\<%
\\
%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}%
\>[7]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Context}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{variable}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaGeneralizable{Θ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\<%
\\
\>[0]\AgdaKeyword{variable}\AgdaSpace{}%
\AgdaGeneralizable{P}\AgdaSpace{}%
\AgdaGeneralizable{Q}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\end{code}
%</context>
\begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{variable}\AgdaSpace{}%
\AgdaGeneralizable{I}\AgdaSpace{}%
\AgdaGeneralizable{J}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\\
\>[0]\<%
\end{code}
%<*forall>
\begin{code}%
\>[0]\AgdaOperator{\AgdaFunction{∀[\AgdaUnderscore{}]}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{I}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\\
\>[0]\AgdaOperator{\AgdaFunction{∀[}}\AgdaSpace{}%
\AgdaBound{P}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{i}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{P}\AgdaSpace{}%
\AgdaBound{i}\<%
\end{code}
%</forall>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaKeyword{infixl}\AgdaSpace{}%
\AgdaNumber{5}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}⊢\AgdaUnderscore{}}}\<%
\end{code}
%<*update>
\begin{code}%
\>[0]\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}⊢\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{I}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{J}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{J}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{I}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaSymbol{(}\AgdaBound{f}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⊢}}\AgdaSpace{}%
\AgdaBound{P}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{i}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{P}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{i}\AgdaSymbol{)}\<%
\end{code}
%</update>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaKeyword{infixr}\AgdaSpace{}%
\AgdaNumber{3}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}⇒\AgdaUnderscore{}}}\<%
\end{code}
%<*arrow>
\begin{code}%
\>[0]\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}⇒\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{P}\AgdaSpace{}%
\AgdaBound{Q}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{I}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{I}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaSymbol{(}\AgdaBound{P}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaBound{Q}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{i}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{P}\AgdaSpace{}%
\AgdaBound{i}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{Q}\AgdaSpace{}%
\AgdaBound{i}\<%
\end{code}
%</arrow>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaKeyword{infixr}\AgdaSpace{}%
\AgdaNumber{4}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∩\AgdaUnderscore{}}}\<%
\end{code}
%<*product>
\begin{code}%
\>[0]\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∩\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{P}\AgdaSpace{}%
\AgdaBound{Q}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{I}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{I}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaSymbol{(}\AgdaBound{P}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∩}}\AgdaSpace{}%
\AgdaBound{Q}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{i}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{P}\AgdaSpace{}%
\AgdaBound{i}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaBound{Q}\AgdaSpace{}%
\AgdaBound{i}\<%
\end{code}
%</product>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{PRINTONLY}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{swapType}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{P}\AgdaSpace{}%
\AgdaBound{Q}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\\
%
\>[2]\AgdaFunction{swapType}\AgdaSpace{}%
\AgdaBound{P}\AgdaSpace{}%
\AgdaBound{Q}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\end{code}
%<*swaptype>
\begin{code}%
\>[2][@{}l@{\AgdaIndent{1}}]%
\>[4]\AgdaOperator{\AgdaFunction{∀[}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},}}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⊢}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{P}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∩}}\AgdaSpace{}%
\AgdaBound{Q}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaBound{Q}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∩}}\AgdaSpace{}%
\AgdaBound{P}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\<%
\end{code}
%</swaptype>
\begin{code}%
\>[0]\<%
\\
%
\>[2]\AgdaFunction{\AgdaUnderscore{}}%
\>[166I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{P}\AgdaSpace{}%
\AgdaBound{Q}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{swapType}\AgdaSpace{}%
\AgdaBound{P}\AgdaSpace{}%
\AgdaBound{Q}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaSymbol{(}\<%
\end{code}
%<*swaptypenormalised>
\begin{code}%
\>[.][@{}l@{}]\<[166I]%
\>[4]\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Γ}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{P}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaBound{Q}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Q}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaBound{P}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{))}\<%
\end{code}
%</swaptypenormalised>
\begin{code}%
%
\>[4]\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{P}\AgdaSpace{}%
\AgdaBound{Q}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\<%
\end{code}
%<*varnormalised>
\begin{code}%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaInductiveConstructor{here}%
\>[11]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Γ}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[32]\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaInductiveConstructor{there}%
\>[11]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Γ}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaBound{Γ}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[32]\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSymbol{)}\<%
\end{code}
%</varnormalised>
\begin{code}%
\>[0]\<%
\\
\>[0]\<%
\end{code}
%<*var>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{here}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∀[}}%
\>[23]\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⊢}}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\<%
\\
%
\>[2]\AgdaInductiveConstructor{there}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∀[}}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}%
\>[23]\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},}}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⊢}}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\<%
\end{code}
%</var>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{PRINTONLY2}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0]\<%
\end{code}
  %<*termdecl>
  \begin{code}%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\end{code}
  %</termdecl>
  %<*termvar>
  \begin{code}%
\>[2][@{}l@{\AgdaIndent{1}}]%
\>[4]\AgdaInductiveConstructor{`var}%
\>[10]\AgdaSymbol{:}%
\>[270I]\AgdaOperator{\AgdaFunction{∀[}}%
\>[16]\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\<%
\\
\>[270I][@{}l@{\AgdaIndent{0}}]%
\>[13]\AgdaComment{--------}\<%
\\
\>[13][@{}l@{\AgdaIndent{0}}]%
\>[16]\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\<%
\end{code}
  %</termvar>
  %<*termapp>
  \begin{code}%
%
\>[4]\AgdaInductiveConstructor{`app}%
\>[10]\AgdaSymbol{:}%
\>[275I]\AgdaOperator{\AgdaFunction{∀[}}%
\>[16]\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\<%
\\
\>[275I][@{}l@{\AgdaIndent{0}}]%
\>[13]\AgdaComment{------------------------}\<%
\\
\>[13][@{}l@{\AgdaIndent{0}}]%
\>[16]\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\<%
\end{code}
  %</termapp>
  %<*termlam>
  \begin{code}%
%
\>[4]\AgdaInductiveConstructor{`lam}%
\>[10]\AgdaSymbol{:}%
\>[285I]\AgdaOperator{\AgdaFunction{∀[}}%
\>[16]\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⊢}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\<%
\\
\>[285I][@{}l@{\AgdaIndent{0}}]%
\>[13]\AgdaComment{----------------}\<%
\\
\>[13][@{}l@{\AgdaIndent{0}}]%
\>[16]\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\<%
\end{code}
  %</termlam>
  \begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\<%
\end{code}
%<*term>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{`var}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∀[}}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\<%
\\
%
\>[2]\AgdaInductiveConstructor{`app}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∀[}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\<%
\\
%
\>[2]\AgdaInductiveConstructor{`lam}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∀[}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⊢}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\<%
\end{code}
%</term>
\begin{code}%
\>[0]\<%
\\
\>[0]\<%
\end{code}
%<*id>
\begin{code}%
\>[0]\AgdaFunction{`id}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∀[}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\<%
\\
\>[0]\AgdaFunction{`id}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSymbol{)}\<%
\end{code}
%</id>
\begin{code}%
\>[0]\AgdaKeyword{infix}\AgdaSpace{}%
\AgdaNumber{0}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\<%
\end{code}
%<*ope>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{done}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\<%
\\
%
\>[2]\AgdaInductiveConstructor{keep}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaGeneralizable{A}%
\>[25]\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaGeneralizable{A}\<%
\\
%
\>[2]\AgdaInductiveConstructor{drop}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{Γ}%
\>[25]\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaGeneralizable{A}\<%
\end{code}
%</ope>
\begin{code}%
\>[0]\<%
\\
\>[0]\<%
\end{code}
%<*lerefl>
\begin{code}%
\>[0]\AgdaFunction{≤-refl}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\<%
\end{code}
%</lerefl>
\begin{code}%
\>[0]\AgdaFunction{≤-refl}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaInductiveConstructor{ε}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{done}\<%
\\
\>[0]\AgdaFunction{≤-refl}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaFunction{≤-refl}\<%
\end{code}

%<*weaken>
\begin{code}%
\>[0]\AgdaFunction{Weaken}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\\
\>[0]\AgdaFunction{Weaken}\AgdaSpace{}%
\AgdaBound{P}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Γ}\AgdaSpace{}%
\AgdaBound{Δ}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaBound{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{P}\AgdaSpace{}%
\AgdaBound{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{P}\AgdaSpace{}%
\AgdaBound{Δ}\<%
\end{code}
%</weaken>
\begin{code}%
\>[0]\<%
\\
\>[0]\<%
\end{code}
%<*weakVar>
\begin{code}%
\>[0]\AgdaFunction{wkVar}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Weaken}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{wkVar}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSymbol{)}%
\>[16]\AgdaBound{v}%
\>[27]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{wkVar}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{wkVar}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSymbol{)}%
\>[16]\AgdaInductiveConstructor{here}%
\>[27]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\<%
\\
\>[0]\AgdaFunction{wkVar}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSymbol{)}%
\>[16]\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}%
\>[27]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{wkVar}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\<%
\end{code}
%</weakVar>
\begin{code}%
\>[0]\<%
\\
\>[0]\<%
\end{code}
%<*weakTerm>
\begin{code}%
\>[0]\AgdaFunction{wkTerm}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Weaken}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{wkTerm}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}%
\>[21]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{wkVar}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{wkTerm}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}%
\>[21]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{wkTerm}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{wkTerm}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{wkTerm}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaBound{b}\AgdaSymbol{)}%
\>[21]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{wkTerm}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{b}\AgdaSymbol{)}\<%
\end{code}
%</weakTerm>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaKeyword{infixr}\AgdaSpace{}%
\AgdaNumber{3}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}`∘\AgdaUnderscore{}}}\<%
\end{code}
%<*composition>
\begin{code}%
\>[0]\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}`∘\AgdaUnderscore{}}}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∀[}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{B}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{C}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{C}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\<%
\\
\>[0]\AgdaBound{g}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{`∘}}\AgdaSpace{}%
\AgdaBound{f}%
\>[8]\AgdaSymbol{=}%
\>[11]\AgdaKeyword{let}\AgdaSpace{}%
\AgdaBound{Γ≤Γ,A}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaFunction{≤-refl}\AgdaSpace{}%
\AgdaKeyword{in}\<%
\\
%
\>[11]\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}%
\>[486I]\AgdaSymbol{(}\AgdaFunction{wkTerm}\AgdaSpace{}%
\AgdaBound{Γ≤Γ,A}\AgdaSpace{}%
\AgdaBound{g}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[486I]%
\>[22]\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{wkTerm}\AgdaSpace{}%
\AgdaBound{Γ≤Γ,A}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSymbol{)))}\<%
\end{code}
%</composition>
\begin{code}%
\>[0]\<%
\\
\>[0]\<%
\end{code}
%<*box>
\begin{code}%
\>[0]\AgdaKeyword{record}\AgdaSpace{}%
\AgdaRecord{□}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Γ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{constructor}\AgdaSpace{}%
\AgdaInductiveConstructor{mk□}\<%
\\
%
\>[2]\AgdaKeyword{field}\AgdaSpace{}%
\AgdaField{run□}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∀[}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤\AgdaUnderscore{}}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\<%
\end{code}
%</box>
\begin{code}%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{□}\<%
\\
\>[0]\<%
\end{code}
%<*kripke>
\begin{code}%
\>[0]\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{P}\AgdaSpace{}%
\AgdaBound{Q}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaBound{P}\AgdaSpace{}%
\AgdaBound{Q}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaRecord{□}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{P}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaBound{Q}\AgdaSymbol{)}\<%
\end{code}
%</kripke>
\begin{code}%
\>[0]\<%
\\
\>[0]\<%
\end{code}
%<*letrans>
\begin{code}%
\>[0]\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Θ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Θ}\<%
\end{code}
%</letrans>
\begin{code}%
\>[0]\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaInductiveConstructor{done}\AgdaSpace{}%
\AgdaInductiveConstructor{done}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{done}\<%
\\
\>[0]\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaBound{p}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaBound{p}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\<%
\\
\>[0]\<%
\end{code}
%<*extract>
\begin{code}%
\>[0]\AgdaFunction{extract}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∀[}}\AgdaSpace{}%
\AgdaRecord{□}\AgdaSpace{}%
\AgdaGeneralizable{P}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaGeneralizable{P}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\<%
\\
\>[0]\AgdaFunction{extract}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{run□}\AgdaSpace{}%
\AgdaFunction{≤-refl}\<%
\end{code}
%</extract>
\begin{code}%
\>[0]\<%
\\
\>[0]\<%
\end{code}
%<*duplicate>
\begin{code}%
\>[0]\AgdaFunction{duplicate}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∀[}}\AgdaSpace{}%
\AgdaRecord{□}\AgdaSpace{}%
\AgdaGeneralizable{P}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaRecord{□}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaRecord{□}\AgdaSpace{}%
\AgdaGeneralizable{P}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\<%
\\
\>[0]\AgdaFunction{duplicate}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{run□}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{run□}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{run□}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∘}}\AgdaSpace{}%
\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaBound{σ}\<%
\end{code}
%</duplicate>
\begin{code}%
\>[0]\<%
\\
\>[0]\<%
\end{code}
%<*weakKripke>
\begin{code}%
\>[0]\AgdaFunction{wkKripke}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Weaken}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaGeneralizable{P}\AgdaSpace{}%
\AgdaGeneralizable{Q}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{wkKripke}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{duplicate}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{run□}\AgdaSpace{}%
\AgdaBound{σ}\<%
\end{code}
%</weakKripke>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ application}\<%
\end{code}
%<*semapp>
\begin{code}%
\>[0]\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}\$\$\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∀[}}\AgdaSpace{}%
\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaGeneralizable{P}\AgdaSpace{}%
\AgdaGeneralizable{Q}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaGeneralizable{P}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaGeneralizable{Q}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\<%
\\
\>[0]\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}\$\$\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{extract}\<%
\end{code}
%</semapp>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ lambda-abstraction}\<%
\\
\>[0]\AgdaKeyword{infixr}\AgdaSpace{}%
\AgdaNumber{3}\AgdaSpace{}%
\AgdaInductiveConstructor{mk□}\<%
\end{code}
%<*mkbox>
\begin{code}%
\>[0]\AgdaKeyword{syntax}\AgdaSpace{}%
\AgdaInductiveConstructor{mk□}\AgdaSpace{}%
\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{b}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{λλ[}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaInductiveConstructor{,}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaInductiveConstructor{]}\AgdaSpace{}%
\AgdaBound{b}\<%
\end{code}
%</mkbox>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ Model\ construction}\<%
\\
\>[0]\AgdaComment{--\ Here\ we\ would\ traditionally\ enforce\ that\ (Value\ `α)}\<%
\\
\>[0]\AgdaComment{--\ returns\ neutral\ terms}\<%
\end{code}
%<*value>
\begin{code}%
\>[0]\AgdaFunction{Value}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\\
\>[0]\AgdaFunction{Value}\AgdaSpace{}%
\AgdaInductiveConstructor{`α}%
\>[16]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{`α}\<%
\\
\>[0]\AgdaFunction{Value}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{)}%
\>[16]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Value}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Value}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{)}\<%
\end{code}
%</value>
\begin{code}%
\>[0]\<%
\\
\>[0]\<%
\end{code}
%<*weakValue>
\begin{code}%
\>[0]\AgdaFunction{wkValue}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Weaken}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Value}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{wkValue}\AgdaSpace{}%
\AgdaInductiveConstructor{`α}%
\>[18]\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{wkTerm}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
\>[0]\AgdaFunction{wkValue}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{)}%
\>[18]\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{wkKripke}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\<%
\end{code}
%</weakValue>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaKeyword{interleaved}\AgdaSpace{}%
\AgdaKeyword{mutual}\<%
\\
\>[0]\<%
\end{code}
%<*reify>
\begin{code}%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaFunction{reify}%
\>[11]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∀[}}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaBound{A}%
\>[38]\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaBound{A}%
\>[49]\AgdaOperator{\AgdaFunction{]}}\<%
\end{code}
%</reify>
\begin{code}%
%
\>[2]\AgdaFunction{reflect}%
\>[11]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∀[}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaBound{A}%
\>[38]\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaBound{A}%
\>[49]\AgdaOperator{\AgdaFunction{]}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\>[2]\AgdaFunction{reify}%
\>[11]\AgdaInductiveConstructor{`α}\AgdaSpace{}%
\AgdaBound{T}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{T}\<%
\\
%
\>[2]\AgdaFunction{reflect}%
\>[11]\AgdaInductiveConstructor{`α}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\>[2]\AgdaFunction{reify}%
\>[11]\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{T}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`lam}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaKeyword{let}%
\>[9]\AgdaBound{f}%
\>[12]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{wkKripke}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaFunction{≤-refl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{T}\<%
\\
%
\>[9]\AgdaBound{v}%
\>[12]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{reflect}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaKeyword{in}\AgdaSpace{}%
\AgdaFunction{reify}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{f}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\$\$}}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaFunction{reflect}%
\>[11]\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{λλ[}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaInductiveConstructor{,}\AgdaSpace{}%
\AgdaBound{V}\AgdaSpace{}%
\AgdaInductiveConstructor{]}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaKeyword{let}%
\>[9]\AgdaBound{f}%
\>[12]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{wkTerm}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
%
\>[9]\AgdaBound{v}%
\>[12]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{reify}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{V}\<%
\\
%
\>[4]\AgdaKeyword{in}\AgdaSpace{}%
\AgdaFunction{reflect}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Type\ of\ environments\ mapping\ variables\ to\ values}\<%
\end{code}
%<*env>
\begin{code}%
\>[0]\AgdaKeyword{record}\AgdaSpace{}%
\AgdaRecord{Env}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Γ}\AgdaSpace{}%
\AgdaBound{Δ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{field}\AgdaSpace{}%
\AgdaField{get}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{A}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{Δ}\<%
\end{code}
%</env>
\begin{code}%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{Env}\<%
\\
\>[0]\<%
\end{code}
%<*extend>
\begin{code}%
\>[0]\AgdaFunction{extend}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∀[}}\AgdaSpace{}%
\AgdaRecord{Env}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaRecord{□}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Value}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaRecord{Env}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\<%
\\
\>[0]\AgdaFunction{extend}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{run□}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{get}\AgdaSpace{}%
\AgdaInductiveConstructor{here}%
\>[35]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
\>[0]\AgdaFunction{extend}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{run□}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{get}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}%
\>[35]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{wkValue}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{get}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\<%
\end{code}
%</extend>
\begin{code}%
\>[0]\<%
\\
\>[0]\<%
\end{code}
%<*eval>
%<*evaldecl>
\begin{code}%
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{Env}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\<%
\end{code}
%</evaldecl>
\begin{code}%
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{get}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\$\$}}\AgdaSpace{}%
\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaBound{b}\AgdaSymbol{)}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{λλ[}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaInductiveConstructor{,}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaInductiveConstructor{]}\AgdaSpace{}%
\AgdaFunction{eval}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{extend}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{run□}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{b}\<%
\end{code}
%</eval>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaFunction{init}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{Env}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\<%
\\
\>[0]\AgdaFunction{init}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{get}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{reflect}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{norm}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\<%
\\
\>[0]\AgdaFunction{norm}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{reify}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∘}}\AgdaSpace{}%
\AgdaFunction{eval}\AgdaSpace{}%
\AgdaFunction{init}\<%
\end{code}
\begin{code}%
\>[0]\AgdaFunction{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{norm}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{A}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`α}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaInductiveConstructor{`α}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{Γ}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{`id}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{`∘}}\AgdaSpace{}%
\AgdaFunction{`id}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaFunction{`id}\<%
\\
\>[0]\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\end{code}


==> TwoTT.tex <==
\begin{code}%
\>[0]\AgdaSymbol{\{-\#}\AgdaSpace{}%
\AgdaKeyword{OPTIONS}\AgdaSpace{}%
\AgdaPragma{--safe}\AgdaSpace{}%
\AgdaPragma{--without-K}\AgdaSpace{}%
\AgdaSymbol{\#-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{------------------------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ The\ content\ of\ this\ module\ is\ based\ on\ the\ paper}\<%
\\
\>[0]\AgdaComment{--\ Staged\ compilation\ with\ two-level\ type\ theory}\<%
\\
\>[0]\AgdaComment{--\ by\ András\ Kovács}\<%
\\
\>[0]\AgdaComment{--\ https://dl.acm.org/doi/abs/10.1145/3547641}\<%
\\
\>[0]\AgdaComment{--}\<%
\\
\>[0]\AgdaComment{--\ and\ some\ classic\ techniques\ to\ represent\ intrinsically-typed\ calculi}\<%
\\
\>[0]\AgdaComment{------------------------------------------------------------------------}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{TwoTT}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Function.Base}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∘\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{id}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{const}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Unary}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{IUniversal}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}⇒\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}⊢\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∩\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{------------------------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ We\ have\ two\ phases:\ source\ code\ and\ staged\ code}\<%
\\
\>[0]\<%
\end{code}
%<*phase>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Phase}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{stg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Phase}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{variable}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Phase}\<%
\end{code}
%</phase>

\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{------------------------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ We\ have\ two\ stages:\ static\ and\ dynamic}\<%
\\
\>[0]\<%
\end{code}
%<*stage>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Phase}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\<%
\\
%
\>[2]\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaGeneralizable{ph}\<%
\end{code}
%</stage>

%<*stagevariables>
\begin{code}%
\>[0]\AgdaKeyword{variable}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaGeneralizable{ph}\<%
\end{code}
%</stagevariables>

\begin{code}%
\>[0]\AgdaComment{------------------------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ Types\ are\ indexed\ by\ the\ stage\ they\ are\ defined\ at}\<%
\\
\>[0]\AgdaComment{--}\<%
\\
\>[0]\AgdaComment{--\ (⇑\ A)\ is\ the\ static\ representation\ of\ a\ dynamic\ type\ A;\ that\ is}\<%
\\
\>[0]\AgdaComment{--\ to\ say\ it\ is\ morally\ the\ type\ of\ metaprograms\ returning\ code\ of}\<%
\\
\>[0]\AgdaComment{--\ type\ A.}\<%
\\
\>[0]\AgdaComment{--}\<%
\\
\>[0]\AgdaComment{--\ Function\ types\ are\ homogeneous:\ both\ domains\ and\ codomains\ need\ to}\<%
\\
\>[0]\AgdaComment{--\ live\ at\ the\ same\ stage.}\<%
\\
\>[0]\AgdaComment{--}\<%
\\
\>[0]\AgdaComment{--\ Pairs\ are\ only\ for\ static\ data.\ This\ is\ a\ feature\ of\ 2\ level\ TT}\<%
\\
\>[0]\AgdaComment{--\ that\ was\ already\ highlighted\ in\ András'\ paper:\ the\ two\ levels\ do}\<%
\\
\>[0]\AgdaComment{--\ not\ need\ to\ have\ the\ same\ features!}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{infixr}\AgdaSpace{}%
\AgdaNumber{10}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}`×\AgdaUnderscore{}}}\<%
\\
\>[0]\AgdaKeyword{infixr}\AgdaSpace{}%
\AgdaNumber{5}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}`⇒\AgdaUnderscore{}}}\<%
\\
\>[0]\<%
\end{code}
%<*types>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{`α}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaGeneralizable{st}\<%
\end{code}
%<*typesnat>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{`ℕ}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaGeneralizable{st}\<%
\end{code}
%</typesnat>
\begin{code}%
%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{`⇑\AgdaUnderscore{}}}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaInductiveConstructor{src}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\<%
\\
%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}`⇒\AgdaUnderscore{}}}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaGeneralizable{st}\<%
\end{code}
%<*typesprod>
\begin{code}%
%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}`×\AgdaUnderscore{}}}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\<%
\end{code}
%</typesprod>
\begin{code}%
\>[0]\<%
\end{code}
%</types>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaKeyword{variable}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaGeneralizable{st}\<%
\\
%
\>[2]\AgdaGeneralizable{B}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaGeneralizable{st}\<%
\\
%
\>[2]\AgdaGeneralizable{C}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaGeneralizable{st}\<%
\\
\>[0]\<%
\end{code}
%<*asStaged>
\begin{code}%
\>[0]\AgdaFunction{asStaged}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaInductiveConstructor{src}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaInductiveConstructor{stg}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\<%
\\
\>[0]\AgdaFunction{asStaged}\AgdaSpace{}%
\AgdaInductiveConstructor{`α}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`α}\<%
\\
\>[0]\AgdaFunction{asStaged}\AgdaSpace{}%
\AgdaInductiveConstructor{`ℕ}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`ℕ}\<%
\\
\>[0]\AgdaFunction{asStaged}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{)}%
\>[19]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{asStaged}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaFunction{asStaged}\AgdaSpace{}%
\AgdaBound{B}\<%
\end{code}
%</asStaged>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{------------------------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ Context\ are\ your\ usual\ left-nested\ lists\ of\ types.}\<%
\\
\>[0]\AgdaComment{--\ Note\ the\ existential\ quantification\ over\ the\ stage\ of\ the\ freshly}\<%
\\
\>[0]\AgdaComment{--\ bound\ variable\ in\ the\ snoc\ case}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{infixl}\AgdaSpace{}%
\AgdaNumber{4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}\<%
\\
\>[0]\<%
\end{code}
%<*context>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{ε}%
\>[7]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\<%
\\
%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}%
\>[7]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Context}\<%
\end{code}
%</context>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaKeyword{variable}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaGeneralizable{θ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{------------------------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ Thinnings}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{infix}\AgdaSpace{}%
\AgdaNumber{0}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\<%
\\
\>[0]\<%
\end{code}
%<*thin>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{done}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\<%
\\
%
\>[2]\AgdaInductiveConstructor{keep}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaGeneralizable{A}\<%
\\
%
\>[2]\AgdaInductiveConstructor{drop}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaGeneralizable{A}\<%
\end{code}
%</thin>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{θ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{θ}\<%
\\
\>[0]\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaInductiveConstructor{done}\AgdaSpace{}%
\AgdaInductiveConstructor{done}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{done}\<%
\\
\>[0]\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaBound{p}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaBound{p}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\<%
\\
\>[0]\<%
\end{code}
%<*thinrefl>
\begin{code}%
\>[0]\AgdaFunction{≤-refl}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Γ}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaBound{Γ}\<%
\\
\>[0]\AgdaFunction{≤-refl}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaInductiveConstructor{ε}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{done}\<%
\\
\>[0]\AgdaFunction{≤-refl}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaFunction{≤-refl}\<%
\end{code}
%</thinrefl>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{------------------------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ Variables\ (could\ be\ defined\ as\ thinning\ from\ a\ singleton\ list)}\<%
\\
\>[0]\<%
\end{code}
%<*var>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{here}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}%
\>[23]\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⊢}}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaInductiveConstructor{there}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}%
\>[23]\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},}}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⊢}}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaFunction{]}\<%
\end{code}
%</var>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaFunction{weak-Var}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\<%
\\
\>[0]\AgdaFunction{weak-Var}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Var}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{weak-Var}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\<%
\\
\>[0]\AgdaFunction{weak-Var}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Var}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{------------------------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ Terms\ are\ indexed\ both\ by\ the\ stage\ of\ the\ type\ of\ the\ computation}\<%
\\
\>[0]\AgdaComment{--\ they\ describe\ but\ also\ by\ a\ boolean\ describing\ whether\ it\ is\ legal}\<%
\\
\>[0]\AgdaComment{--\ to\ uses\ quotes\ and\ splices}\<%
\\
\>[0]\<%
\end{code}
%<*term>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ph}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Phase}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaBound{ph}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{`var}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaInductiveConstructor{`app}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaInductiveConstructor{`lam}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⊢}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{]}\<%
\end{code}
%<*termnat>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{`zero}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaInductiveConstructor{`ℕ}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaInductiveConstructor{`succ}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaInductiveConstructor{`ℕ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaInductiveConstructor{`ℕ}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaInductiveConstructor{`iter}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`ℕ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{]}\<%
\end{code}
%</termnat>
\begin{code}%
%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{`⟨\AgdaUnderscore{}⟩}}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`⇑}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{`∼\AgdaUnderscore{}}}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`⇑}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaFunction{]}\<%
\end{code}
%<*termprod>
\begin{code}%
%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}`,\AgdaUnderscore{}}}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}%
\>[15]\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\<%
\\
%
\>[15]\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`×}}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaInductiveConstructor{`fst}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{((}\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`×}}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
%
\>[2]\AgdaInductiveConstructor{`snd}%
\>[9]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{((}\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`×}}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{]}\<%
\end{code}
%</termprod>
\begin{code}%
\>[0]\<%
\end{code}
%</term>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ Action\ of\ thinnings\ on\ terms}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Var}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaBound{b}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{keep}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{b}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaInductiveConstructor{`zero}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`zero}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`succ}\AgdaSpace{}%
\AgdaBound{n}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`succ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{n}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaInductiveConstructor{`iter}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`iter}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`∼}}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`∼}}\AgdaSpace{}%
\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`,}}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`,}}\AgdaSpace{}%
\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaInductiveConstructor{`fst}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`fst}\<%
\\
\>[0]\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaInductiveConstructor{`snd}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`snd}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{------------------------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ Example\ of\ programs}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Purely\ dynamic\ identity\ function}\<%
\end{code}
%<*iddyn>
\begin{code}%
\>[0]\AgdaFunction{`idᵈ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\<%
\\
\>[0]\AgdaFunction{`idᵈ}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSymbol{)}\<%
\end{code}
%</iddyn>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ Static\ identity\ function}\<%
\end{code}
%<*idsta>
\begin{code}%
\>[0]\AgdaFunction{`idˢ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\<%
\\
\>[0]\AgdaFunction{`idˢ}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSymbol{)}\<%
\end{code}
%</idsta>
\begin{code}%
\>[0]\<%
\\
\>[0]\<%
\end{code}
%<*composition>
\begin{code}%
\>[0]\AgdaKeyword{infixr}\AgdaSpace{}%
\AgdaNumber{3}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}`∘\AgdaUnderscore{}}}\<%
\\
\>[0]\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}`∘\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{B}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{C}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaGeneralizable{C}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
\>[0]\AgdaBound{g}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{`∘}}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaSymbol{=}%
\>[10]\AgdaKeyword{let}\AgdaSpace{}%
\AgdaBound{Γ≤Γ,A}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaFunction{≤-refl}\AgdaSpace{}%
\AgdaKeyword{in}\<%
\\
%
\>[10]\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{Γ≤Γ,A}\AgdaSpace{}%
\AgdaBound{g}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{Γ≤Γ,A}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSymbol{)))}\<%
\end{code}
%</composition>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ Turning\ static\ nats\ into\ dyanmic\ ones\ by\ computing\ their}\<%
\\
\>[0]\AgdaComment{--\ representation\ as\ codes}\<%
\end{code}
%<*reify>
\begin{code}%
\>[0]\AgdaFunction{`reify}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`ℕ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇑}}\AgdaSpace{}%
\AgdaInductiveConstructor{`ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
\>[0]\AgdaFunction{`reify}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaInductiveConstructor{`iter}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSymbol{))}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[3]\AgdaSymbol{(}\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaInductiveConstructor{`succ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`∼}}\AgdaSpace{}%
\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSymbol{))}\<%
\\
%
\>[3]\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaInductiveConstructor{`zero}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSymbol{)}\<%
\end{code}
%</reify>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ Addition\ in\ terms\ of\ iteration}\<%
\end{code}
%<*add>
\begin{code}%
\>[0]\AgdaFunction{`add}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`ℕ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaInductiveConstructor{`ℕ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaInductiveConstructor{`ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
\>[0]\AgdaFunction{`add}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaInductiveConstructor{`iter}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`succ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSymbol{))))}\<%
\end{code}
%</add>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ Double\ as\ addition\ of\ a\ term\ with\ itself.}\<%
\\
\>[0]\AgdaComment{--\ Note\ that\ we\ return\ a\ *dynamic*\ value\ which\ will\ have\ been}\<%
\\
\>[0]\AgdaComment{--\ computed\ at\ staging\ time}\<%
\\
\>[0]\AgdaFunction{`double}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`ℕ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇑}}\AgdaSpace{}%
\AgdaInductiveConstructor{`ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\<%
\\
\>[0]\AgdaFunction{`double}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaFunction{`reify}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaFunction{`add}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSymbol{)))}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Efficiently\ computing\ the\ Fibonacci\ sequence\ using\ a\ pair}\<%
\\
\>[0]\AgdaComment{--\ of\ values.\ aux(n)\ =\ (fib\ n,\ fib\ (suc\ n))}\<%
\end{code}
%<*fib>
\begin{code}%
\>[0]\AgdaFunction{`fib}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`ℕ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaInductiveConstructor{`ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\<%
\\
\>[0]\AgdaFunction{`fib}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`fst}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{`∘}}\AgdaSpace{}%
\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaComment{--\ this\ implements\ n\ ↦\ (fib\ n,\ fib\ (1\ +\ n))}\<%
\\
%
\>[2]\AgdaInductiveConstructor{`iter}%
\>[678I]\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSymbol{))}\<%
\\
\>[.][@{}l@{}]\<[678I]%
\>[8]\AgdaComment{\{-\ step\ -\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`lam}\<%
\\
\>[8][@{}l@{\AgdaIndent{0}}]%
\>[10]\AgdaKeyword{let}%
\>[681I]\AgdaBound{fibₙ}%
\>[22]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaInductiveConstructor{`fst}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[681I]%
\>[14]\AgdaBound{fib₁₊ₙ}%
\>[22]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaInductiveConstructor{`snd}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSymbol{)}\<%
\\
%
\>[14]\AgdaBound{fib₂₊ₙ}%
\>[22]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaFunction{`add}\AgdaSpace{}%
\AgdaBound{fibₙ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{fib₁₊ₙ}\<%
\\
%
\>[10]\AgdaKeyword{in}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{fib₁₊ₙ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`,}}\AgdaSpace{}%
\AgdaBound{fib₂₊ₙ}\AgdaSymbol{)))}\<%
\\
%
\>[8]\AgdaComment{\{-\ base\ -\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`zero}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`,}}\AgdaSpace{}%
\AgdaInductiveConstructor{`succ}\AgdaSpace{}%
\AgdaInductiveConstructor{`zero}\AgdaSymbol{))}\<%
\end{code}
%</fib>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{------------------------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ Semantics\ toolkit:\ Kripke\ function\ spaces\ between}\<%
\\
\>[0]\AgdaComment{--\ context-indexed\ type\ families}\<%
\\
\>[0]\<%
\end{code}
%<*kripke>
\begin{code}%
\>[0]\AgdaKeyword{record}\AgdaSpace{}%
\AgdaRecord{□}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Γ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{constructor}\AgdaSpace{}%
\AgdaInductiveConstructor{mkBox}\<%
\\
%
\>[2]\AgdaKeyword{field}\AgdaSpace{}%
\AgdaField{runBox}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Δ}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaBound{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{Δ}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Γ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\\
\>[0]\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaRecord{□}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{)}\<%
\end{code}
%</kripke>
\begin{code}%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{□}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Action\ of\ thinnings\ on\ Kripke\ functions\ spaces}\<%
\\
\>[0]\AgdaComment{--\ By\ construction\ they're\ the\ Free\ thinnable}\<%
\\
\>[0]\AgdaFunction{weak-Kripke}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\<%
\\
\>[0]\AgdaFunction{weak-Kripke}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{runBox}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{runBox}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∘}}\AgdaSpace{}%
\AgdaFunction{≤-trans}\AgdaSpace{}%
\AgdaBound{σ}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ lambda-abstraction}\<%
\\
\>[0]\AgdaKeyword{infixr}\AgdaSpace{}%
\AgdaNumber{3}\AgdaSpace{}%
\AgdaInductiveConstructor{mkBox}\<%
\\
\>[0]\AgdaKeyword{syntax}\AgdaSpace{}%
\AgdaInductiveConstructor{mkBox}\AgdaSpace{}%
\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{b}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{λλ[}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaInductiveConstructor{,}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaInductiveConstructor{]}\AgdaSpace{}%
\AgdaBound{b}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ application}\<%
\end{code}
%<*kripkeapp>
\begin{code}%
\>[0]\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}\$\$\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\<%
\\
\>[0]\AgdaBound{f}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\$\$}}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{runBox}\AgdaSpace{}%
\AgdaFunction{≤-refl}\AgdaSpace{}%
\AgdaBound{t}\<%
\end{code}
%</kripkeapp>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{------------------------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ Definition\ of\ the\ domain\ for\ staging\ by\ evaluation}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Empty}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{⊥}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat.Base}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{ℕ}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{suc}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaPrimitive{\AgdaUnderscore{}+\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\AgdaSpace{}%
\AgdaSymbol{as}\AgdaSpace{}%
\AgdaModule{Prod}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}×\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\<%
\end{code}
%<*modelstadecl>
\begin{code}%
\>[0]\AgdaFunction{Static}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\end{code}
%</modelstadecl>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ Static\ values\ are\ intepreted\ in\ the\ domain,}\<%
\\
\>[0]\AgdaComment{--\ Dynamic\ ones\ will\ become\ staged\ terms}\<%
\end{code}
%<*model>
\begin{code}%
\>[0]\AgdaFunction{Value}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\\
\>[0]\AgdaFunction{Value}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}%
\>[11]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{Static}\<%
\\
\>[0]\AgdaFunction{Value}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}%
\>[11]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{stg}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∘}}\AgdaSpace{}%
\AgdaFunction{asStaged}\<%
\end{code}
%</model>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ This\ is\ a\ fairly\ standard\ Kripke\ domain}\<%
\end{code}
%<*modelsta>
\begin{code}%
\>[0]\AgdaFunction{Static}\AgdaSpace{}%
\AgdaInductiveConstructor{`α}%
\>[17]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{const}\AgdaSpace{}%
\AgdaFunction{⊥}\<%
\end{code}
%<*modelnat>
\begin{code}%
\>[0]\AgdaFunction{Static}\AgdaSpace{}%
\AgdaInductiveConstructor{`ℕ}%
\>[17]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{const}\AgdaSpace{}%
\AgdaDatatype{ℕ}\<%
\end{code}
%</modelnat>
\begin{code}%
\>[0]\AgdaFunction{Static}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`⇑}}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{)}%
\>[17]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaBound{A}\<%
\\
\>[0]\AgdaFunction{Static}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{)}%
\>[17]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Static}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Static}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{)}\<%
\end{code}
%<*modelprod>
\begin{code}%
\>[0]\AgdaFunction{Static}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`×}}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{)}%
\>[17]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{Static}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∩}}\AgdaSpace{}%
\AgdaFunction{Static}\AgdaSpace{}%
\AgdaBound{B}\<%
\end{code}
%</modelprod>
%</modelsta>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ Action\ of\ thinnings\ on\ Kripke\ domains}\<%
\\
\>[0]\AgdaFunction{weak-Static}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Static}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Static}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\<%
\\
\>[0]\AgdaFunction{weak-Static}\AgdaSpace{}%
\AgdaInductiveConstructor{`α}%
\>[21]\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{id}\<%
\\
\>[0]\AgdaFunction{weak-Static}\AgdaSpace{}%
\AgdaInductiveConstructor{`ℕ}%
\>[21]\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{id}\<%
\\
\>[0]\AgdaFunction{weak-Static}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`⇑}}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{)}%
\>[21]\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\<%
\\
\>[0]\AgdaFunction{weak-Static}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{weak-Kripke}\AgdaSpace{}%
\AgdaBound{σ}\<%
\\
\>[0]\AgdaFunction{weak-Static}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`×}}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{Prod.map}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Static}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Static}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Action\ of\ thinnings\ on\ Values}\<%
\\
\>[0]\AgdaFunction{weak-Value}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\<%
\\
\>[0]\AgdaFunction{weak-Value}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{st}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{weak-Static}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
\>[0]\AgdaFunction{weak-Value}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{st}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{weak-Term}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{------------------------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ Evaluator\ for\ staging\ by\ evaluation}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Type\ of\ environments\ mapping\ variables\ to\ values}\<%
\\
\>[0]\AgdaKeyword{record}\AgdaSpace{}%
\AgdaRecord{Env}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Γ}\AgdaSpace{}%
\AgdaBound{Δ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Context}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{field}\AgdaSpace{}%
\AgdaField{lookup}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{st}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Var}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{Δ}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{Env}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Action\ of\ thinnings\ on\ environments}\<%
\\
\>[0]\AgdaComment{--\ (pointwise\ lifting\ of\ the\ action\ on\ values)}\<%
\\
\>[0]\AgdaFunction{weak-Env}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaGeneralizable{θ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Env}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Env}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaGeneralizable{θ}\<%
\\
\>[0]\AgdaFunction{weak-Env}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{lookup}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{A}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{weak-Value}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{lookup}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Semantics\ counterpart\ to\ iter}\<%
\end{code}
%<*iter>
\begin{code}%
\>[0]\AgdaFunction{iterate}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{ty}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ty}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{ty}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{ty}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{ty}\<%
\\
\>[0]\AgdaFunction{iterate}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{z}\AgdaSpace{}%
\AgdaNumber{0}%
\>[21]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{z}\<%
\\
\>[0]\AgdaFunction{iterate}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{z}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{n}\AgdaSymbol{)}%
\>[21]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{iterate}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{z}\AgdaSpace{}%
\AgdaBound{n}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{iter}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{A}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`ℕ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\<%
\\
\>[0]\AgdaFunction{iter}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}%
\>[10]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`iter}\<%
\\
\>[0]\AgdaFunction{iter}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}%
\>[10]\AgdaSymbol{=}%
\>[1064I]\AgdaInductiveConstructor{λλ[}\AgdaSpace{}%
\AgdaBound{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaInductiveConstructor{,}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaInductiveConstructor{]}\AgdaSpace{}%
\AgdaInductiveConstructor{λλ[}\AgdaSpace{}%
\AgdaBound{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaInductiveConstructor{,}\AgdaSpace{}%
\AgdaBound{succ}\AgdaSpace{}%
\AgdaInductiveConstructor{]}\AgdaSpace{}%
\AgdaInductiveConstructor{λλ[}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaInductiveConstructor{,}\AgdaSpace{}%
\AgdaBound{zero}\AgdaSpace{}%
\AgdaInductiveConstructor{]}\<%
\\
\>[.][@{}l@{}]\<[1064I]%
\>[12]\AgdaFunction{iterate}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weak-Kripke}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{succ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\$\$\AgdaUnderscore{}}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{zero}\AgdaSpace{}%
\AgdaBound{m}\<%
\end{code}
%</iter>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ Semantics\ counterpart\ to\ app}\<%
\end{code}
%<*app>
\begin{code}%
\>[0]\AgdaFunction{app}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\<%
\\
\>[0]\AgdaFunction{app}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}%
\>[9]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}\$\$\AgdaUnderscore{}}}\<%
\\
\>[0]\AgdaFunction{app}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}%
\>[9]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`app}\<%
\end{code}
%</app>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ Extending\ an\ environment\ with\ a\ value\ to\ push\ it\ under\ a\ binder}\<%
\end{code}
%<*extend>
\begin{code}%
\>[0]\AgdaFunction{extend}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaRecord{Env}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaRecord{□}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Value}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⇒}}\AgdaSpace{}%
\AgdaRecord{Env}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
\>[0]\AgdaFunction{extend}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{runBox}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{lookup}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
\>[0]\AgdaFunction{extend}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{runBox}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{lookup}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{A}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{weak-Value}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{lookup}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\<%
\\
\>[0]\<%
\end{code}
%</extend>
\begin{code}%
\>[0]\<%
\\
\>[0]\<%
\end{code}
%<*lam>
\begin{code}%
\>[0]\AgdaFunction{lam}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[1152I]\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaBound{st}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
\>[.][@{}l@{}]\<[1152I]%
\>[6]\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Value}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Value}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
%
\>[6]\AgdaFunction{Value}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⇒}}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\<%
\\
\>[0]\AgdaFunction{lam}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}%
\>[9]\AgdaBound{b}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{λλ[}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaInductiveConstructor{,}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaInductiveConstructor{]}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{runBox}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
\>[0]\AgdaFunction{lam}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}%
\>[9]\AgdaBound{b}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{b}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{runBox}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{drop}\AgdaSpace{}%
\AgdaFunction{≤-refl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaInductiveConstructor{here}\AgdaSymbol{))}\<%
\end{code}
%</lam>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ Semantics\ counterpart\ to\ zero}\<%
\end{code}
%<*zero>
\begin{code}%
\>[0]\AgdaFunction{zero}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaInductiveConstructor{`ℕ}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\<%
\\
\>[0]\AgdaFunction{zero}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}%
\>[10]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaNumber{0}\<%
\\
\>[0]\AgdaFunction{zero}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}%
\>[10]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`zero}\<%
\end{code}
%</zero>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ Semantics\ counterpart\ to\ succ}\<%
\end{code}
%<*succ>
\begin{code}%
\>[0]\AgdaFunction{succ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Stage}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaInductiveConstructor{`ℕ}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaInductiveConstructor{`ℕ}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\<%
\\
\>[0]\AgdaFunction{succ}\AgdaSpace{}%
\AgdaInductiveConstructor{sta}%
\>[10]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaOperator{\AgdaPrimitive{+\AgdaUnderscore{}}}\<%
\\
\>[0]\AgdaFunction{succ}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}%
\>[10]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`succ}\<%
\end{code}
%</succ>

%<*bodydecl>
\begin{code}%
\>[0]\AgdaFunction{body}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[1230I]\AgdaRecord{Env}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
\>[.][@{}l@{}]\<[1230I]%
\>[7]\AgdaFunction{Kripke}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Value}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Value}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\<%
\end{code}
%</bodydecl>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ Evaluation\ function\ turning\ src\ terms\ into\ values\ provided}\<%
\\
\>[0]\AgdaComment{--\ we\ have\ an\ environment\ assigning\ values\ to\ variables}\<%
\end{code}
%<*evaldecl>
\begin{code}%
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{Env}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{Γ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Value}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaGeneralizable{Δ}\<%
\end{code}
%</evaldecl>
%<*eval>
\begin{code}%
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`var}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}%
\>[29]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{lookup}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{st}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{st}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}%
\>[29]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{app}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`lam}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{st}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{st}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{b}\AgdaSymbol{)}%
\>[29]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{lam}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{body}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{b}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`zero}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{st}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{st}\AgdaSymbol{\})}%
\>[29]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{zero}\AgdaSpace{}%
\AgdaBound{st}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`succ}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{st}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{st}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{n}\AgdaSymbol{)}%
\>[29]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{succ}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{n}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`iter}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{st}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{st}\AgdaSymbol{\})}%
\>[29]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{iter}\AgdaSpace{}%
\AgdaBound{st}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}%
\>[29]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`∼}}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}%
\>[29]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{v}\<%
\end{code}
%<*evalprod>
\begin{code}%
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`,}}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}%
\>[29]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaInductiveConstructor{`fst}%
\>[29]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{λλ[}\AgdaSpace{}%
\AgdaBound{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaInductiveConstructor{,}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaInductiveConstructor{]}\AgdaSpace{}%
\AgdaField{Prod.proj₁}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
\>[0]\AgdaFunction{eval}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaInductiveConstructor{`snd}%
\>[29]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{λλ[}\AgdaSpace{}%
\AgdaBound{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaInductiveConstructor{,}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaInductiveConstructor{]}\AgdaSpace{}%
\AgdaField{Prod.proj₂}\AgdaSpace{}%
\AgdaBound{v}\<%
\end{code}
%</evalprod>
%</eval>

%<*body>
\begin{code}%
\>[0]\AgdaFunction{body}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{λλ[}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaInductiveConstructor{,}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaInductiveConstructor{]}\AgdaSpace{}%
\AgdaFunction{eval}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{extend}\AgdaSpace{}%
\AgdaBound{ρ}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{runBox}\AgdaSpace{}%
\AgdaBound{σ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{b}\<%
\end{code}
%</body>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ Special\ case\ of\ evaluation:\ turning\ source\ terms\ into\ staged\ ones}\<%
\\
\>[0]\<%
\end{code}
%<*stagedecl>
\begin{code}%
\>[0]\AgdaFunction{stage}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{stg}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{asStaged}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\<%
\end{code}
%</stagedecl>
\begin{code}%
\>[0]\AgdaFunction{stage}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{eval}\AgdaSpace{}%
\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaKeyword{where}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{lookup}\AgdaSpace{}%
\AgdaSymbol{())}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≡\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{------------------------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ Tests\ for\ the\ staging\ evaluator}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{infix}\AgdaSpace{}%
\AgdaNumber{0}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∋\AgdaUnderscore{}↝\AgdaUnderscore{}}}\<%
\\
\>[0]\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∋\AgdaUnderscore{}↝\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{src}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaInductiveConstructor{stg}\AgdaSpace{}%
\AgdaInductiveConstructor{dyn}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{asStaged}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{ε}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\\
\>[0]\AgdaBound{A}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∋}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{↝}}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{stage}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ `idˢ\ is\ a\ static\ identity\ and\ thus\ computes}\<%
\\
\>[0]\AgdaFunction{test-idˢ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaInductiveConstructor{`ℕ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∋}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`∼}}\AgdaSpace{}%
\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaFunction{`idˢ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaInductiveConstructor{`zero}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{↝}}\AgdaSpace{}%
\AgdaInductiveConstructor{`zero}\<%
\\
\>[0]\AgdaFunction{test-idˢ}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ `idᵈ\ is\ a\ dynamic\ identity\ and\ thus\ stays\ stuck}\<%
\\
\>[0]\AgdaFunction{test-idᵈ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaInductiveConstructor{`ℕ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∋}}\AgdaSpace{}%
\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaFunction{`idᵈ}\AgdaSpace{}%
\AgdaInductiveConstructor{`zero}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{↝}}\AgdaSpace{}%
\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaFunction{`idᵈ}\AgdaSpace{}%
\AgdaInductiveConstructor{`zero}\<%
\\
\>[0]\AgdaFunction{test-idᵈ}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ We\ can\ of\ course\ mix\ the\ two}\<%
\\
\>[0]\AgdaFunction{test-idᵈˢ}%
\>[1458I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{stage}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaFunction{`idᵈ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`∼}}\AgdaSpace{}%
\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaFunction{`idˢ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`⟨}}\AgdaSpace{}%
\AgdaInductiveConstructor{`zero}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSymbol{))}\<%
\\
\>[.][@{}l@{}]\<[1458I]%
\>[10]\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaFunction{`idᵈ}\AgdaSpace{}%
\AgdaInductiveConstructor{`zero}\<%
\\
\>[0]\AgdaFunction{test-idᵈˢ}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Just\ for\ ease\ of\ use\ in\ the\ test\ cases\ involving\ computations}\<%
\\
\>[0]\AgdaFunction{fromℕ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{∀[}\AgdaSpace{}%
\AgdaDatatype{Term}\AgdaSpace{}%
\AgdaGeneralizable{ph}\AgdaSpace{}%
\AgdaGeneralizable{st}\AgdaSpace{}%
\AgdaInductiveConstructor{`ℕ}\AgdaSpace{}%
\AgdaFunction{]}\<%
\\
\>[0]\AgdaFunction{fromℕ}\AgdaSpace{}%
\AgdaInductiveConstructor{ℕ.zero}%
\>[16]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`zero}\<%
\\
\>[0]\AgdaFunction{fromℕ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ℕ.suc}\AgdaSpace{}%
\AgdaBound{n}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{`succ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{fromℕ}\AgdaSpace{}%
\AgdaBound{n}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{test-add}\AgdaSpace{}%
\AgdaSymbol{:}\<%
\end{code}
%<*testadd>
\begin{code}%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaInductiveConstructor{`ℕ}%
\>[6]\AgdaOperator{\AgdaFunction{∋}}%
\>[9]\AgdaOperator{\AgdaInductiveConstructor{`∼}}\AgdaSpace{}%
\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaFunction{`reify}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaFunction{`add}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{fromℕ}\AgdaSpace{}%
\AgdaNumber{7}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{fromℕ}\AgdaSpace{}%
\AgdaNumber{35}\AgdaSymbol{))}\<%
\\
%
\>[6]\AgdaOperator{\AgdaFunction{↝}}%
\>[9]\AgdaFunction{fromℕ}\AgdaSpace{}%
\AgdaNumber{42}\<%
\end{code}
%</testadd>
\begin{code}%
\>[0]\AgdaFunction{test-add}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Finally,\ the\ static\ `double\ computes\ at\ staging\ time}\<%
\\
\>[0]\AgdaFunction{test-double}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaInductiveConstructor{`ℕ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∋}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{`∼}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaFunction{`double}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{fromℕ}\AgdaSpace{}%
\AgdaNumber{4}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{↝}}\AgdaSpace{}%
\AgdaFunction{fromℕ}\AgdaSpace{}%
\AgdaNumber{8}\<%
\\
\>[0]\AgdaFunction{test-double}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ And\ computing\ fib\ by\ using\ pairs,\ a\ feature\ not\ available}\<%
\\
\>[0]\AgdaComment{--\ in\ the\ target\ language!}\<%
\\
\>[0]\AgdaFunction{test-fib}\AgdaSpace{}%
\AgdaSymbol{:}\<%
\end{code}
%<*testfib>
\begin{code}%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaInductiveConstructor{`ℕ}%
\>[1517I]\AgdaOperator{\AgdaFunction{∋}}%
\>[8]\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaFunction{`add}\AgdaSpace{}%
\AgdaInductiveConstructor{`zero}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{`∼}}\AgdaSpace{}%
\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{`reify}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{`∘}}\AgdaSpace{}%
\AgdaFunction{`fib}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{fromℕ}\AgdaSpace{}%
\AgdaNumber{8}\AgdaSymbol{))}\<%
\\
\>[.][@{}l@{}]\<[1517I]%
\>[5]\AgdaOperator{\AgdaFunction{↝}}%
\>[8]\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{`app}\AgdaSpace{}%
\AgdaFunction{`add}\AgdaSpace{}%
\AgdaInductiveConstructor{`zero}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{fromℕ}\AgdaSpace{}%
\AgdaNumber{21}\AgdaSymbol{)}\<%
\end{code}
%</testfib>
\begin{code}%
\>[0]\AgdaFunction{test-fib}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%


==> robust-catch.tex <==
\makeatletter

\newrobustcmd*\OrigExecuteMetaData[2][\jobname]{%
\CatchFileBetweenTags\CatchFBT@tok{#1}{#2}%
\global\expandafter\CatchFBT@tok\expandafter{%
\expandafter}\the\CatchFBT@tok
}%\OrigExecuteMetaData

\newrobustcmd*\ChkExecuteMetaData[2][\jobname]{%
\CatchFileBetweenTags\CatchFBT@tok{#1}{#2}%
\edef\mytokens{\detokenize\expandafter{\the\CatchFBT@tok}}
\ifx\mytokens\empty\PackageError{catchfilebetweentags}{the tag #2 is not found\MessageBreak in file #1 \MessageBreak called from \jobname.tex}{use a different tag}\fi%
}%\ChkExecuteMetaData

\renewrobustcmd*\ExecuteMetaData[2][\jobname]{%
\ChkExecuteMetaData[#1]{#2}%
\OrigExecuteMetaData[#1]{#2}%
}

\makeatother

